Optimizing Data Collection for Machine Learning

Modern deep learning systems require huge data sets to achieve impressive performance, but there is little guidance on how much or what kind of data to collect. Over-collecting data incurs unnecessary present costs, while under-collecting may incur future costs and delay workflows. We propose a new paradigm for modeling the data collection workflow as a formal optimal data collection problem that allows designers to specify performance targets, collection costs, a time horizon, and penalties for failing to meet the targets. Additionally, this formulation generalizes to tasks requiring multiple data sources, such as labeled and unlabeled data used in semi-supervised learning. To solve our problem, we develop Learn-Optimize-Collect (LOC), which minimizes expected future collection costs. Finally, we numerically compare our framework to the conventional baseline of estimating data requirements by extrapolating from neural scaling laws. We significantly reduce the risks of failing to meet desired performance targets on several classification, segmentation, and detection tasks, while maintaining low total collection costs.

==> How Much More Data Should I Get for ArXiv/macros.tex <==
\newif\ifcomments
% Replace with \commentsfalse to disable comments (e.g. to check submission length)
\commentstrue

\newcommand{\mr}[2]{\multirow{#1}{*}{#2}}%
\newcommand{\fir}[1]{\mathbf{#1}}
\newcommand{\seco}[1]{\underline{#1}}


\newcommand{\authcomment}[3]{\ifcomments {\color{#2} [#1: #3]} \else \fi}

\newcommand{\RRM}[1]{\authcomment{RRM}{blue}{#1}}
\newcommand{\ML}[1]{\authcomment{ML}{cyan}{#1}}
\newcommand{\JL}[1]{\authcomment{JL}{orange}{#1}}
\newcommand{\JA}[1]{\authcomment{JA}{red}{#1}}
\newcommand{\ZY}[1]{\authcomment{ZY}{magenta}{#1}}
\newcommand{\SF}[1]{\authcomment{SF}{green}{#1}}


%\newcommand{\rebut}[1]{{\color{blue}{#1}}}
\newcommand{\rebut}[1]{{#1}}

==> How Much More Data Should I Get for ArXiv/sections/abstract.tex <==
\begin{abstract}
%Modern deep learning systems require huge datasets to achieve their impressive performance, but there is little guidance available on how much data should be collected to train a deep learning system to meet some target performance. 
%Determining the correct data collection budget is critical. 
%Over-estimation incurs excess costs while under-estimation may incur future costs, workflow delays, or, in the worst case, identify a project as infeasible only after the data deficit is realized. 
Modern deep learning systems require huge data sets to achieve impressive performance, but there is little guidance on how much or what kind of data to collect. Over-collecting data incurs unnecessary present costs, while under-collecting may incur future costs and delay workflows. We propose a new paradigm for modeling the data collection workflow as a formal \emph{optimal data collection problem} that allows designers to specify performance targets, collection costs, a time horizon, and penalties for failing to meet the targets. Additionally, this formulation generalizes to tasks requiring multiple data sources, such as labeled and unlabeled data used in semi-supervised learning. To solve our problem, we develop Learn-Optimize-Collect (LOC), which minimizes expected future collection costs. Finally, we numerically compare our framework to the conventional baseline of estimating data requirements by extrapolating from neural scaling laws. We significantly reduce the risks of failing to meet desired performance targets on several classification, segmentation, and detection tasks, while maintaining low total collection costs.
\end{abstract}


==> How Much More Data Should I Get for ArXiv/sections/app_experiment_results.tex <==
%\clearpage
\section{Additional Numerical Results}
\label{sec:app_experiment_results}



This section contains expanded results of our numerical experiments and further ablations. Our key results include:
%

$\bullet$ In Appendix~\ref{sec:app_estimating_data_requirement_distribution}, we evaluate the effectiveness of estimating $F(q)$ by plotting the estimated learning curves as well as the empirical histograms used to model the data requirement distribution.
    

$\bullet$  In Appendix~\ref{sec:app_experiment_robustness}, we explore the sensitivity of our optimization algorithm to variations in the cost and penalty parameters. In all except one instance, LOC consistently maintains a low total cost and failure rate.
    
$\bullet$  In Appendix~\ref{sec:app_experiment_k_equals_two}, we explore the multi-variate LOC (i.e., $K=2$) for problems where we have a small number of $T=1, 3$ rounds. The baseline fails for almost all instances of $T=1$, whereas LOC maintains a low failure rate.
    
$\bullet$  In Appendix~\ref{sec:app_experiment_alternate_regression_functions}, we consider variants of LOC where we use different regression functions to estimate the data requirement distribution. Our optimization framework can be deployed on top of any regression function to reduce the failure rate.
    





\rebut{

\subsection{Estimating the Data Requirement Distribution $F(q)$}
\label{sec:app_estimating_data_requirement_distribution}


To estimate $F(q)$, we first create an ensemble of estimated learning curves, which we then invert to obtain an empirical distribution of estimated values for $D^*$.
Figure~\ref{fig:app_learning_curves} plots our bootstrap resampled estimated learning curves versus the ground truth performance for the first round of data collection when we have access to an initial $\dataset_{q_0}$ containing $10\%$ of the full data set. 
As noted in~\citet{mahmood2022howmuch}, the mean estimated learning curve diverges from the ground truth. 
However, by bootstrap resampling an ensemble of learning curves, we can cover the ground truth with some probability.


Figure~\ref{fig:app_histograms} plots the empirical histograms of estimated $D^*$ as well as the estimated $F(q)$ obtained via KDE on CIFAR-10 with three different values for $V^*$.
Although the mode of the estimated distribution is far from the ground truth $D^*$, the estimated distribution assigns some probability to the ground truth region. 
LOC optimizes over this estimated $F(q)$, which allows us to conservatively collect data and reduce the chances of failure.
}





\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/regress/CIFAR-10_powerlaw_bootstrap_seed_3_n_5.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/regress/CIFAR-100_powerlaw_bootstrap_seed_3_n_5.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/regress/ImageNet_powerlaw_bootstrap_seed_4_n_4.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/regress/VOC_powerlaw_bootstrap_seed_4_n_2.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/regress/BDD100K_powerlaw_bootstrap_seed_3_n_5.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/regress/nuScenes_powerlaw_bootstrap_seed_1_n_5.pdf}\end{minipage}
%
\vspace{-3mm}
\caption{\label{fig:app_learning_curves}
\rebut{
For a fixed seed, ground truth learning curves (black) and the estimated power law learning curves (blue) obtained via bootstrapping and ensembling. The shaded region represents the $95$ percentile of the ensemble and the dashed blue line represents the mean of the regression functions. The mean is consistently higher than the unknown ground truth, whereas the shaded region can at times cover it.
}
}
\end{center}
\vspace{-4mm}
%\vspace{-8mm}
%\vspace{-9mm}
\end{figure*}





\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.30\linewidth}\includegraphics[width=1\textwidth]{figures/regress/big_CIFAR-100_powerlaw_bootstrap_seed_3_n_5_50_Hist.pdf}\end{minipage}
\begin{minipage}{0.30\linewidth}\includegraphics[width=1\textwidth]{figures/regress/big_CIFAR-100_powerlaw_bootstrap_seed_3_n_5_60_Hist.pdf}\end{minipage}
\begin{minipage}{0.30\linewidth}\includegraphics[width=1\textwidth]{figures/regress/big_CIFAR-100_powerlaw_bootstrap_seed_3_n_5_70_Hist.pdf}\end{minipage}
%
\vspace{-3mm}
\caption{\label{fig:app_histograms}
\rebut{
For a fixed seed, the histogram of estimates of $D^*$ from different bootstrapped models (blue bars), the estimated $F(q)$ (orange curve), and the ground truth $D^*$ (black dashed line). 
Each plot corresponds to a different $V^*$ for CIFAR-100 (see Figure~\ref{fig:app_learning_curves} for the learning curve). 
With higher targets, regression (i.e., collecting the mean of the distribution) will lead to larger under-estimations.
}
}
\end{center}
\vspace{-4mm}
\end{figure*}
















\subsection{Robustness to the Cost and Penalty Parameters}
\label{sec:app_experiment_robustness}



\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t1_V2/sweepcost_cifar10_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t1_V2/sweepcost_cifar100_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t1_V2/sweepcost_imagenet_powerlawbootstrap_1_1.pdf}\end{minipage}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t3_V2/sweepcost_cifar10_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t3_V2/sweepcost_cifar100_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t3_V2/sweepcost_imagenet_powerlawbootstrap_3_1.pdf}\end{minipage}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t1_V2/sweepcost_voc_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t1_V2/sweepcost_bdd100k_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t1_V2/sweepcost_liftsplatshoot_powerlawbootstrap_1_1.pdf}\end{minipage}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t3_V2/sweepcost_voc_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t3_V2/sweepcost_bdd100k_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t3_V2/sweepcost_liftsplatshoot_powerlawbootstrap_3_1.pdf}\end{minipage}
%
\vspace{-3mm}
\caption{\label{fig:app_sweep_cost}
Mean $\pm$ standard deviation of the ratio of data collected $q_T^* / D^*$ for different $V^*$ when we sweep the cost parameter from $0.001$ to $1$ and fix $P=10^7$. 
We show $T=1, 3$ and refer to the main paper for $T=5$.
The dashed black line corresponds to collecting exactly the minimum data requirement.
%See Appendix~\ref{sec:app_experiment_results} for results on all $T$.
}
\end{center}
\vspace{-4mm}
%\vspace{-9mm}
\end{figure*}






\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t1_V2/sweepcost_cifar10_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t1_V2/sweepcost_cifar100_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t1_V2/sweepcost_imagenet_powerlawbootstrap_1_1.pdf}\end{minipage}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t3_V2/sweepcost_cifar10_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t3_V2/sweepcost_cifar100_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t3_V2/sweepcost_imagenet_powerlawbootstrap_3_1.pdf}\end{minipage}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t1_V2/sweepcost_voc_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t1_V2/sweepcost_bdd100k_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t1_V2/sweepcost_liftsplatshoot_powerlawbootstrap_1_1.pdf}\end{minipage}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t3_V2/sweepcost_voc_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t3_V2/sweepcost_bdd100k_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t3_V2/sweepcost_liftsplatshoot_powerlawbootstrap_3_1.pdf}\end{minipage}
%
\vspace{-3mm}
\caption{\label{fig:app_sweep_penalty}
Mean $\pm$ std of the ratio of data collected $q_T^* / D^*$ for different $V^*$ when we sweep the penalty parameter from $10^6$ to $10^9$ and fix $c=1$. 
We show $T=1, 3$ and refer to the main paper for $T=5$.
The dashed black line corresponds to collecting exactly the minimum data requirement.
%See Appendix~\ref{sec:app_experiment_results} for results on all $T$.
}
\end{center}
\vspace{-4mm}
%\vspace{-8mm}
%\vspace{-9mm}
\end{figure*}






Figure~\ref{fig:app_sweep_cost} expands the cost parameter sweep from Figure~\ref{fig:sweep_cost_and_penalty} (Top row) to the settings of $T=1, 3$. For nearly all settings, LOC remains stable to variations in the cost parameter. 
Nonetheless, careful parameter selection becomes important as $T$ decreases.
This is due to the fact that for low costs, the total amount of data collected increases as $T$ decreases (e.g., $c = 0.001$ for BDD100K).
Furthermore, Figure~\ref{fig:app_sweep_penalty} expands the penalty parameter sweep from Figure~\ref{fig:sweep_cost_and_penalty} (Bottom row). 
Here, we observe similar properties to the cost parameter sweep.




Although LOC is relatively stable on all other data sets, our results demonstrate some extreme results for VOC, potentially due to noise in the simulation. For example in Figure~\ref{fig:app_sweep_penalty}, setting $P=10^9$, $V^*=71$, and $T=3$ led to collecting $10,000$ times the minimum data requirement. 
Such a situation is unrealistic in a production-level implementation, since in a real implementation, we could impose further constraints onto problem~\eqref{eq:expected_risk_prob}, such as upper bounds on the total amount of data permissible.

















\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t1_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_1_1,0.5_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t1_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_1_1,0.2_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t1_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_1_1,0.1_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t1_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_1_1,0.05_0_100000000.0.pdf} \end{minipage}
%
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t3_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_3_1,0.5_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t3_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_3_1,0.2_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t3_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_3_1,0.1_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t3_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_3_1,0.05_0_100000000.0.pdf} \end{minipage}
%
\vspace{-4mm}
\caption{\label{fig:app_head_to_head_two_d_cifar}
%\RRM{These results are raw and I am running another set with more trials.}
For experiments on CIFAR-100 with two data types, mean $\pm$ standard deviation over 5 seeds of the cost ratio $\bc^\tpose (\bq^*_T - \bq_0) / \bc^\tpose (\bD^* - \bq_0) - 1$ and failure rate for different $V$ after removing $99$-th percentile outliers. 
We fix $c_0=1$ and $P=10^{13}$.
The rows correspond to $T=1, 3$ (see the main paper for $T=5$) and the columns correspond to $c_1 = c_0/2, c_0/5, c_0/10, c_0/20$. 
%See Appendix~\ref{sec:app_experiment_k_equals_2} for all $T$.
}
\end{center}
\vspace{-4mm}
%\vspace{-8mm}
%\vspace{-9mm}
\end{figure*}





\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t1_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_1_1,0.1_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t1_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_1_1,0.05_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t1_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_1_1,0.01_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t1_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_1_1,0.005_0_1000000000.0.pdf} \end{minipage}
%
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t3_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_3_1,0.1_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t3_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_3_1,0.05_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t3_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_3_1,0.01_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t3_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_3_1,0.005_0_1000000000.0.pdf} \end{minipage}
%
%
\vspace{-4mm}
\caption{\label{fig:app_head_to_head_two_d_bdd}
%\RRM{These results are raw and I am running another set with more trials.}
For experiments on BDD100K with two data types, mean $\pm$ standard deviation over 5 seeds of the cost ratio $\bc^\tpose (\bq^*_T - \bq_0) / \bc^\tpose (\bD^* - \bq_0) - 1$ and failure rate for different $V$ after removing $99$-th percentile outliers. 
We fix $c_0=1$ and $P=10^{13}$.
The rows correspond to $T=1, 3$ (see the main paper for $T=5$) and the columns correspond to $c_1 = c_0/2, c_0/5, c_0/10, c_0/20$. 
%See Appendix~\ref{sec:app_experiment_k_equals_2} for all $T$.
}
\end{center}
\vspace{-4mm}
%\vspace{-8mm}
%\vspace{-9mm}
\end{figure*}




\subsection{The Value of Optimization over Estimation when $K = 2$}
\label{sec:app_experiment_k_equals_two}



Figure~\ref{fig:app_head_to_head_two_d_cifar} and Figure~\ref{fig:app_head_to_head_two_d_bdd} expand Figure~\ref{fig:two_d_head_to_head} to $T=1, 3$ rounds. The results validate the summary observations from Table~\ref{tab:two_d_summary} in that the baseline has considerably higher failure rates versus LOC. In particular for BDD100K at $T=1$, the baseline fails consistently for four out of five random seeds. 
On the other hand, recall that LOC admits a higher cost ratio compared to the baseline when $T=1$. We can observe now that this high cost ratio is due to the method incurring high cost for a few target $V^*$ values. 
This behavior is similar to the observation above on VOC with high penalties at $T=3$. 









\begin{table}[!t]
    \centering
%\begin{minipage}{0.75\linewidth}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
  Regression Function   &  $T$ & \multicolumn{2}{c}{Regression} & \multicolumn{2}{c}{LOC} \\ \cmidrule(lr){3-4}\cmidrule(lr){5-6}
           &      & Failure rate & Cost ratio & Failure rate & Cost ratio \\
\midrule
\multirow{3}{*}{Logarithmic $\hat{v}(q;\btheta) = \theta_0 \log (q + \theta_1) + \theta_2$}
  &  1 &                $43\%$ &                 $0.19$ &              $\fir{2\%}$ &               $1.17$ \\
  &  3 &                $37\%$ &                 $0.17$ &              $\fir{2\%}$ &               $0.54$ \\
  &  5 &                $34\%$ &                 $0.16$ &              $\fir{1\%}$ &               $0.39$ \\
\midrule
\multirow{3}{*}{Arctan $\hat{v}(q;\btheta) = \frac{200}{\pi} \arctan (\theta_0 \frac{\pi}{2} q + \theta_1) + \theta_2$}
  &  1 &                $23\%$ &                 $3.31$ &               $\fir{0\%}$ &               $5.56$ \\
  &  3 &                $15\%$ &                 $3.01$ &               $\fir{0\%}$ &               $3.92$ \\
  &  5 &                $12\%$ &                 $2.90$ &               $\fir{0\%}$ &               $3.60$ \\
 \midrule
\multirow{3}{*}{Algebraic Root $\hat{v}(q;\btheta) = \frac{100 q}{1 + | \theta_0 q |^{\theta_1})^{1/\theta_1}} +  \theta_2$}
  & \rebut{ 1 } &               \rebut{ $52\%$ } &              \rebut{   $0.11$ } &            \rebut{  $\fir{23\%}$ } &               \rebut{ $0.81$ }  \\
  & \rebut{ 3 } &               \rebut{ $44\%$ } &              \rebut{    $0.1$ } &            \rebut{   $\fir{2\%}$ } &               \rebut{ $0.87$ } \\
  & \rebut{ 5 } &               \rebut{ $44\%$ } &              \rebut{    $0.1$ } &            \rebut{   $\fir{2\%}$ } &               \rebut{ $0.54$ } \\
\bottomrule
\end{tabular}
}
%\end{minipage}
%
%\hfill
%\begin{minipage}{0.5\linewidth}{}
%\begin{minipage}{0.31\linewidth}
    \caption{For experiments on CIFAR-100, average cost ratio $\bc^\tpose (\bq^*_T - \bq_0) / \bc^\tpose (\bD^* - \bq_0) - 1$ and failure rate measured over a range of $V^*$ and $T$. 
    We fix $c = 1$ and $P=10^7$.
    The best performing failure rate for each setting is bolded. The cost ratio is measured only for instances that achieve $V^*$. LOC consistently reduces the average failure rate, almost consistently down to $0\%$.}
    \label{tab:one_d_other_methods}
%\end{minipage}
\vspace{-5mm}
\end{table}




\begin{table}[!t]
    %\centering
\begin{minipage}{0.69\linewidth}
\rebut{
\resizebox{\linewidth}{!}{
\begin{tabular}{clccccc}
\toprule
  & Data set &  $T$ & \multicolumn{2}{c}{Regression With Correction~\cite{mahmood2022howmuch}} & \multicolumn{2}{c}{LOC} \\ \cmidrule(lr){4-5}\cmidrule(lr){6-7}
  &          &      & Failure rate & Cost ratio & Failure rate & Cost ratio \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{Class.}}    
& \multirow{3}{*}{CIFAR-100}    &  1 &   $      14\%$ &   $\seco{0.94}$ &        $\fir{4\%}$ &    $0.99$ \\
&                               &  3 &   $\fir{ 1\%}$ &   $\seco{0.23}$ &        $     3\% $ &    $0.31$ \\
&                               &  5 &   $\fir{ 0\%}$ &   $\seco{0.17}$ &        $     2\% $ &    $0.19$ \\
  \cmidrule{2-7} 
 & \multirow{3}{*}{Imagenet}    &  1 &   $\fir{ 7\%}$ &          $1.03$ &        $     37\% $ &    $\seco{0.49}$ \\
 &                              &  3 &   $\fir{ 0\%}$ &          $0.21$ &        $      5\% $ &    $\seco{0.16}$ \\
 &                              &  5 &   $\fir{ 0\%}$ &          $0.14$ &        $      2\% $ &    $\seco{0.10}$ \\
 \midrule
  \multirow{6}{*}{\rotatebox[origin=c]{90}{Seg.}}    
  & \multirow{3}{*}{BDD100K}    &  1 &   $\fir{ 4\%}$ &          $4.03$ &        $     12\% $ &    $\seco{2.03}$ \\
  &                             &  3 &   $\fir{ 0\%}$ &          $1.02$ &        $\fir{ 0\%}$ &    $\seco{0.72}$ \\
  &                             &  5 &   $\fir{ 0\%}$ &          $0.62$ &        $\fir{ 0\%}$ &    $\seco{0.35}$ \\
  \cmidrule{2-7} 
 & \multirow{3}{*}{nuScenes}    &  1 &   $\fir{ 0\%}$ &          $27.2$ &        $     52\% $ &    $\seco{0.16}$ \\
 &                              &  3 &   $\fir{ 0\%}$ &          $0.75$ &        $\fir{ 0\%}$ &    $\seco{0.09}$ \\
 &                              &  5 &   $\fir{ 0\%}$ &          $0.30$ &        $\fir{ 0\%}$ &    $\seco{0.04}$ \\
 \midrule
 \multirow{3}{*}{\rotatebox[origin=c]{90}{Det.}}    
      & \multirow{3}{*}{VOC}    &  1 &   $\fir{ 0\%}$ &          $44.6$ &        $     25\% $ &    $\seco{0.56}$ \\
      &                         &  3 &   $\fir{ 0\%}$ &          $7.02$ &        $\fir{ 0\%}$ &    $\seco{1.10}$ \\
      &                         &  5 &   $\fir{ 0\%}$ &          $3.98$ &        $\fir{ 0\%}$ &    $\seco{0.84}$ \\
\bottomrule
\end{tabular}
}
}
\end{minipage}
%
\hfill
%\begin{minipage}{0.5\linewidth}{}
\begin{minipage}{0.28\linewidth}
    \caption{
    \rebut{
    Comparison against the correction factor-based Power Law Regression of~\citet{mahmood2022howmuch} 
    using the same setup as in Table~\ref{tab:one_d_summary}.
    The best performing cost ratio is underlined and the best performing failure rate for each setting is bolded. 
    Although the baseline is designed specifically to achieve low failure rates, LOC often can achieve competitive failure rates while reducing the cost ratios by an order of magnitude.
    }
    }
    \label{tab:one_d_with_tolerance}
\end{minipage}
\vspace{-2mm}
\end{table}







\subsection{LOC with Alternative Regression Functions}
\label{sec:app_experiment_alternate_regression_functions}




\citet{mahmood2022howmuch} show that we can use other regression functions instead of the power law to estimate the data requirement. Moreover, some functions tend to consistently over- or under-estimate the requirement. 
LOC can be deployed on top of any such regression function, since the regression function is only used to generate bootstrap samples.



Table~\ref{tab:one_d_other_methods} highlights experiments on CIFAR-100 with \rebut{three} alternative regression functions that were used by~\citet{mahmood2022howmuch}.
For both functions, we observe the same trends seen in Table~\ref{tab:one_d_summary}. That is, LOC reduces the failure rate down to approximately zero, at a marginal relative increase in cost. 
%Furthermore, note that different regression functions have different downstream performance (e.g., Logarithmic has higher failure rates with lower costs than Arctan). 


\rebut{

Noting that Power Law Regression often leads to failure,~\citet{mahmood2022howmuch} also propose a correction factor heuristic wherein they learn a parameter $\tau$ such that if the data collection problem requires a target performance $V^*$, we should instead aim to collect enough data to meet $V^* + \tau$. 
In order to learn this correction factor, we require a pre-existing data set upon which we can simulate a data collection policy.
\citet{mahmood2022howmuch} suggest setting $\tau$ such that we can achieve the data requirement $V^*$ for any $V^*$ on the pre-existing data set, and then fixing this parameter for new data sets.


Table~\ref{tab:one_d_with_tolerance} compares LOC (i.e., repeating Table~\ref{tab:one_d_summary}) with the Correction factor-based Power Law regression baseline of~\citet{mahmood2022howmuch}. Following the original paper, we tune $\tau$ using CIFAR-10 and apply it on all other data sets. 
The correction factor is designed to minimize the failure rate and thus, achieves nearly $0\%$ failure rate for all settings, but often at high cost ratios. 
On the other hand, LOC achieves generally low failure rates and low cost ratios. Specifically, for $T=3, 5$, we are competitive with the baseline on failure rates for most tasks while obtaining up to an order of magnitude decrease in costs. For $T=1$, we typically admit higher failure rates; however for the segmentation and detection tasks, we obtain up multiple orders of magnitude lower costs.
Finally, note that this baseline requires a similar prior task to be effective. For example, the baseline outperforms us on cost and failure rate both only on CIFAR-100, since it is tuned on CIFAR-10. On the other hand, LOC does not require this prior data set to be effective as evidence by its performance on non-classification tasks.


}




==> How Much More Data Should I Get for ArXiv/sections/app_experiments.tex <==
%\clearpage
\section{Simulation Experiment Setup}
\label{sec:app_experiments}







The most intuitive approach of validating our data collection problem is by repeatedly sampling from a data set, training a model, and solving the optimization problem. However, performing a large set of such experiments over many data sets becomes computationally intractable. 
Instead, we follow the approach introduced in~\citet{mahmood2022howmuch}, which proposes a simulation model of the data collection problem.
This section summarizes the simulation setup.




The simulation replicates the steps in Algorithm~\ref{alg:data_collection} except with one key difference. In the simulation, we replace the score function $V(\dataset)$ with a \emph{ground truth} function $v\gt(q)$ that serves as an oracle which reports the expected score of the model trained with $q$ data points. 
Thus, rather than having to collect data and train a model in each round, we evaluate $v\gt(q_t)$ and treat this as the current model score. 
The optimization and regression models do not have access to $v\gt(q)$.






\subsection{A Piecewise-Linear Ground Truth Approximation}






In order to build a ground truth function, we first use the sub-sampling procedure in Algorithm~\ref{alg:data_collection} to collect performance statistics over subsets of the entire training data set. 
Using these observed statistics, we then build a piecewise-linear model of the ground truth. %Below, we first summarize the data collection process and then the linear model.
Below, we first highlight how to construct a piecewise-linear model when given a set of data set sizes and their corresponding scores. In the next subsection, we will detail the exact data collection process.


\noindent\textbf{The Single-variate ($K=1$) Case.}
\citet{mahmood2022howmuch} develop a ground truth function as follows. Let $q_0 \leq q_1 \leq q_2 \leq \cdots$ be a series of data set sizes and let $\dataset_{q_0} \subset \dataset_{q_1} \subset \dataset_{q_2} \subset \cdots$ be their corresponding sets. Then, consider the following piecewise-linear function:
%
\begin{align*}
    v\gt(q) := \begin{cases} \displaystyle
        \frac{V(\dataset_{q_0})}{q_0} n , & q \leq q_0 \\  \displaystyle
        \frac{V(\dataset_{q_t}) - V(\dataset_{q_{t-1}})}{q_t - q_{t-1}} \left( q - q_t \right) + V(\dataset_{q_{t-1}}), & q_{t-1} \leq q \leq q_t
    \end{cases}
\end{align*}
%
This function is concave and monotonically increasing, which follows the general trend of real learning curves~\cite{hestness2017deep}. Furthermore~\citet{mahmood2022howmuch} show that given sufficient resolution, i.e., enough data subsets, this piecewise linear function is an accurate approximation of the true learning curve $V(\dataset)$.




\noindent\textbf{The Multi-variate $(K=2)$ Case.}
In the previous $K=1$ case, the ground truth was formed by taking linear approximations between different subset sizes. When $K > 1$, we have multiple subsets that are used to evaluate the score $V(\dataset^1, \dots, \dataset^K)$. 



We focus specifically on $K=2$ in our numerical experiments and propose a generalization of the previous piecewise-linear function. Here, rather than building lines on the intervals between subsequent sets, we build planes on triangular intervals. Specifically, let $q^1_0 \leq q^1_1 \leq q^1_2 \leq \cdots$ and  $q^2_0 \leq q^2_1 \leq q^2_2 \leq \cdots$ be two series of data set sizes, and consider the grid 
%
\begin{align*}\begin{array}{cccc}
    (q^1_0, q^2_0)  & (q^1_1, q^2_0)   & (q^1_2, q^2_0)     & \cdots \\
    (q^1_0, q^2_1)  & (q^1_1, q^2_1)   & (q^1_2, q^2_1)     & \cdots \\
    (q^1_0, q^2_2)  & (q^1_1, q^2_2)   & (q^1_2, q^2_2)     & \cdots \\
    \vdots          & \vdots           & \vdots             & \ddots \\
    \end{array}
\end{align*}
%
For each tuple $(q^1_s, q^2_t)$ in the above grid, let $V(\dataset^1_{q^1_s}, \dataset^2_{q^2_t})$ be the score of a model trained on two data sets of the corresponding respective sizes. 




For each index $(s, t)$ we fit linear models on the corresponding lower right and upper left triangles. First, let $(\underline{\alpha}(s, t), \underline{\beta}(s, t), \underline{\gamma}(s, t))$ be the parameters of the plane defined by the lower triangle $\{ (q^1_{s-1}, q^2_t), (q^1_{s}, q^2_{t-1}), (q^1_{s}, q^2_t) \}$, i.e., the unique solution to the following linear system:
%
\begin{align*}
    \begin{pmatrix}
        q^1_{s-1}   & q^2_t      & 1 \\
        q^1_{s}     & q^2_{t-1}  & 1 \\
        q^1_{s}     & q^2_{t}    & 1 \\
    \end{pmatrix}
    \begin{pmatrix}
        \underline{\alpha}(s, t) \\
        \underline{\beta}(s, t) \\
        \underline{\gamma}(s, t)
    \end{pmatrix}
    = 
    \begin{pmatrix}
        V(\dataset^1_{q^1_{s-1}}, \dataset^2_{q^2_t}) \\
        V(\dataset^1_{q^1_{s}}, \dataset^2_{q^2_{t-1}}) \\
        V(\dataset^1_{q^1_{s}}, \dataset^2_{q^2_t}) \\
    \end{pmatrix}
\end{align*}
%
Thus, for any data set sizes $(q^1, q^2)$ in this triangle, we evaluate the ground truth by the linear model $\underline{\alpha}(s, t) q^1 + \underline{\beta}(s, t) q^2 + \underline{\gamma}(s, t)$. 
Similarly, let $(\overline{\alpha}(s, t), \overline{\beta}(s, t), \overline{\gamma}(s, t))$ be the parameters of the plane defined by the upper triangle $\{ (q^1_{s}, q^2_t), (q^1_{s+1}, q^2_{t}), (q^1_{s}, q^2_{t+1}) \}$, i.e., the unique solution to the following linear system:
%
\begin{align*}
    \begin{pmatrix}
        q^1_{s}   & q^2_t        & 1 \\
        q^1_{s+1} & q^2_{t}      & 1 \\
        q^1_{s}   & q^2_{t+1}    & 1 \\
    \end{pmatrix}
    \begin{pmatrix}
        \overline{\alpha}(s, t) \\
        \overline{\beta}(s, t) \\
        \overline{\gamma}(s, t)
    \end{pmatrix}
    = 
    \begin{pmatrix}
        V(\dataset^1_{q^1_{s}}, \dataset^2_{q^2_t}) \\
        V(\dataset^1_{q^1_{s+1}}, \dataset^2_{q^2_{t}}) \\
        V(\dataset^1_{q^1_{s}}, \dataset^2_{q^2_{t+1}}) \\
    \end{pmatrix}
\end{align*}
%
Similarly for any $(q^1, q^2)$ in this triangle, the ground truth is obtained by the linear model $\overline{\alpha}(s, t) q^1 + \overline{\beta}(s, t) q^2 + \overline{\gamma}(s, t)$. 


Finally, we define our ground truth function $v\gt(q^1, q^2)$. For any $q^1 \geq q^1_0, q^2 \geq q^2_0$, this function first identifies the interval $[q^1_s, q^1_{s+1}] \times [q^2_t, q^2_{t+1}]$ in which the point lies. Then, the function assigns a score based on whether the point lies in the upper left or the lower right triangle in this interval. We write this function as
%
\begin{align*}
    v\gt(q^1, q^2) := & \begin{cases} \displaystyle
        \overline{\alpha}(s, t) q^1 + \overline{\beta}(s, t) q^2 + \overline{\gamma}(s, t) \\ \displaystyle
            \qquad\qquad\qquad\qquad\qquad \text{ if } \norm{(q^1, q^2) - (q^1_s, q^2_t)} \leq \norm{(q^1, q^2) - (q^1_{s+1}, q^2_{t+1})}, \\  \displaystyle
        \underline{\alpha}(s+1, t+1) q^1 + \underline{\beta}(s+1, t+1) q^2 + \underline{\gamma}(s+1, t+1) \\
            \qquad\qquad\qquad\qquad\qquad \text{ otherwise},
    \end{cases}
    \\
    & \text{for } q^1_s \leq q^1 \leq q^1_{s+1} \;,\; q^2_t \leq q^2 \leq q^2_{t+1}.
\end{align*}




\begin{table}[t!]
    \centering
    \footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{lll cc}
\toprule
             Data set & Task & Score & \multicolumn{2}{c}{Full data set size} \\
\midrule
    CIFAR-10~\cite{krizhevsky2009learning}  & Classification & Accuracy & \multicolumn{2}{c}{$50,000$}     \\
    CIFAR-100~\cite{krizhevsky2009learning} & Classification & Accuracy & \multicolumn{2}{c}{$50,000$}      \\
    ImageNet~\cite{deng2009imagenet} & Classification & Accuracy & \multicolumn{2}{c}{$1,281,167$}   \\ %\midrule
    BDD100K~\cite{yu2020bdd100k} & Semantic Segmentation & Mean IoU & \multicolumn{2}{c}{$7,000$}          \\
    nuScenes~\cite{nuscenes2019} & BEV Segmentation & Mean IoU & \multicolumn{2}{c}{$28,130$}    \\ %\midrule
    VOC~\cite{pascal-voc-2007, pascal-voc-2012} & 2-D Object Detection & Mean AP & \multicolumn{2}{c}{$16,551$}       \\ 
    %nuScenes~\cite{nuscenes2019} & 3-D Object Detection & Mean AP & $28,130$ \\ \midrule
\midrule
    CIFAR-100~\cite{krizhevsky2009learning} & Classification & Accuracy & $25,000$ (Classes 0-49) & $25,000$ (Classes 50-99) \\
    BDD100K~\cite{yu2020bdd100k} &  Semantic Segmentation & Mean IoU & $7,000$ (Labeled) & $70,000$ (Unlabeled) \\
\bottomrule
\end{tabular}
}
    %\vspace{-1em}
    \caption{Data sets, tasks, and score functions considered.}
    \label{tab:tasks}
    \vspace{-2em}
\end{table}



\rebut{
\noindent\textbf{For $K > 2$.}
The piecewise linear approximations grow increasingly complex as the dimension $K$ increases.
Furthermore, the number of subsets of data set sizes required to create a piecewise linear approximation increases exponentially with $K$. 
Specifically for $k \in \{1,\dots, K\}$, let $M_k$ denote the number of subsets (i.e., $|\{q_0^k, q_1^k, \dots, q_{M_k}^k \}|$) of a data set that we consider when creating subsets. For each combination of $K$ subsets, we must then train a model and evaluate it's performance to record $V(\dataset^1, \dots, \dataset^K)$. Thus, we must subsample and train our model for $O(\prod_{k}M_k)$ combinations. 
This can quickly become computationally prohibitive. %, we avoid experiments for $K > 2$.
}




\subsection{Data Collection}
\label{sec:app_data_collection}



We now summarize the data collection and training process used to create the above piecewise-linear functions for each data set and task.
All models were implemented using PyTorch and trained on machines with up to eight NVIDIA V100 GPU cards. 
Table~\ref{tab:tasks} details each task and data set size.






\noindent\textbf{Image Classification Tasks.} For all experiments with CIFAR-10 and CIFAR-100, we use a ResNet18~\cite{he2016deep} following the same procedure as in~\citet{coleman2019selection}. For ImageNet, we use a ResNet34~\cite{he2016deep} using the procedure in~\citet{coleman2019selection}. 
All models are trained with cross entropy loss using SGD with momentum. We evaluate all models on Top-1 Accuracy.




For all experiments, we set the initial data set at $q_0 = 10\%$ of the data. In data collection, we create five subsets containing $2\%, 4\%, \cdots, 10\%$ of the training data, five subsets containing $12\%, 14\%, \cdots, 20\%$ of the training data, and eight subsets containing $30\%, 40\%, \cdots, 100\%$ of the data. Note that we use higher granularity in the early stage as this is where the dynamics of the learning curve vary the most. With more data, the learning curve eventually has a nearly zero slope.
For each subset, we train our respective model and evaluate performance.



\noindent\textbf{VOC.}
We use the Single-Shot Detector 300 (SSD300)~\cite{liu2016ssd} based on a VGG16 backbone~\cite{simonyan2014very}, following the same procedure as in~\citet{elezi2021towards}. All models are trained using SGD with momentum. We evaluate all models on mean AP.



For all experiments, we set the initial data set at $q_0 = 10\%$ of the data. 
In data collection, we sample twenty subsets at $5\%$ intervals, i.e., $5\%, 10\%, 15\%, \cdots, 100\%$ of the training data.



\noindent\textbf{BDD100K.}
We use Deeplabv3 \cite{chen2017rethinking} with ResNet50 backbone. We use random initialization for the backbone. We use the original data set split from \citet{yu2020bdd100k} with $7,000$ and $1,000$ data points in the train and validation sets respectively. The evaluation metrics is mean Intersection over Union (IoU).
We follow the same protocol used in the Image classification tasks to create our subsets of data.








\noindent\textbf{nuScenes.}
We use the ``Lift Splat'' architecture~\cite{liftsplat}, which is used for BEV segmentation from driving scenes, following the steps from the original paper to train this model. We evaluate on mean IoU. Our data collection procedure follows the same steps and percentages of the data set as used for BDD100K and the Image classification tasks.





\noindent\textbf{CIFAR-100 (2 Types).}
We partition this data set into two subsets $\dataset^1$ and $\dataset^2$ of $25,000$ images each containing the first 50 and last 50 classes, respectively. We then train a ResNet18~\citep{he2016deep} using different fractions of the two subsets. We follow the same training procedure as in the single-variate case except with one difference. Since some of the data sets will naturally be imbalanced (e.g., if we train with half of the first subset and all of the second subset), we employ a class-balanced cross entropy loss using the inverse frequency of samples per class.


For each $\dataset^k$ subsets, respectively, we follow the same subsampling procedure used in the single-variate case. That is, we let $q^1_0 = 10\%$ of the first data subset and $q^2_0 =10\%$ of the second data subset. For each subset, we create $10$ subsampled sets at intervals of $2\%, 4\%, 6\%, \cdots, 20\%$ of the respective data subset. We then create eight further subsampled sets at $30\%, 40\%, \cdots, 100\%$ of the respective data subset.
Finally, we train our model and evaluate the score on every combination of the subsampled subsets of $\dataset^1 \times \dataset^2$. 




\noindent\textbf{BDD100K (Semi-supervised).}
For this task, we consider semi-supervised segmentation via pseudo-labeling the unlabeled data set in BDD100K. The data is partitioned into two subsets $\dataset^1$ and $\dataset^2$ containing $7,000$ labeled and $70,000$ unlabeled scenes. As before, we use the Deeplabv3~\citep{chen2017rethinking} architecture with a ResNet50 backbone. Here however, we:
%
\begin{enumerate}
    \item First train with a labeled subset of $\dataset^1$ via supervised learning.
    \item Pseudo-label an unlabeled subset of $\dataset^2$ using the trained model.
    \item Re-train the model with the labeled subset and the pseudo-labeled subset.
\end{enumerate}
%
We follow the same procedure as in the single-variate case for both training steps, except we weigh the unlabeled data by $0.2$ to reduce its contribution to the loss.



Training via semi-supervised learning on BDD100K requires long compute times, so we reduce the number of subsets used in this experiment. 
For the labeled set $\dataset^1$, we create subsets with $5\%, 10\%, 15\%, 20\%, 40\%, 60\%, 80\%, 100\%$ of the data.
For the unlabeled set $\dataset^2$, we create subsets with $0\%, 10\%, 25\%, 50\%, 100\%$ of the data.
Note that we have five settings of unlabeled data since we include the case of training with no unlabeled data as well. 









\begin{table}[!t]
    \centering
    %\def\arraystretch{1.5}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{p{0.35\linewidth} p{0.65\linewidth}}
        \toprule
        Parameter & Setting \\
        \midrule
        Optimizer   & GD with Momentum ($\beta = 0.9$), Adam ($\beta_0, \beta_1 = 0.9, 0.999$) \\
        Learning rate   & $0.005, \dots, 500$ \\
        Number of bootstrap samples $B$ & $500$ \\
        Number of regression subsets $R$ & See Appendix~\ref{sec:app_data_collection} \\
        Density Estimation Model    & KDE for $K=1$, GMM for $K=2$ \\
        \multirow{2}{*}{KDE Bandwidth}  & $20000, \dots, 20000000$ for ImageNet \\
                                        & $200, \dots, 4000$ for all others \\
        GMM number of clusters          & $4, \dots, 10$ \\   
        \bottomrule
    \end{tabular}
    }
    \caption{Summary of hyperparameters used in our experiments.}
    \label{tab:hyperparameters}
\end{table}





\subsection{LOC Implementation}



For all experiments, we initialize with $10$\% of the training data set. We consider $T=1,3,5$ rounds and sweep a range of $V^*$. We provide a summary of parameters in Table~\ref{tab:hyperparameters}.



For the experiments with $K=1$, we model the data requirement PDF $f(q)$ in each round of the problem as follows. We first draw $B=500$ bootstrap resamples of the current training statistics $\set{R}$, where $\set{R} = \{ (rq_0/R, V(\dataset_{rq_0/R})) \}_{r=1}^R \cup \{ (q_s, V(\dataset_{q_s})) \}_{s=1}^t$ contains all of the measured statistics up to the initial data set (e.g., for CIFAR-10, this includes performance with $2\%, 4\%, \cdots, 10\%$ of the data), and the previous collected data. The latter is obtained by calling our piecewise-linear ground truth approximation. 
For each bootstrap resample, we fit a power regression model $\hat{v}(q;\btheta) = \theta_0 q^{\theta_1} + \theta_2$ and solve for the estimated minimum data requirement. We then use our set of estimates to fit a Kernel Density Estimation (KDE) model after gridsearching for the best bandwidth parameter.



For the experiments with $K=2$, we use the same above procedure but fit Gaussian Mixture Models (GMM) due to their having an easily computable CDF via the Gaussian $\mathrm{erf}(\cdot)$, rather than numerically integrating the PDF.
We grid-search over the number of mixture components for the GMM model.


We optimize over problems~\eqref{eq:expected_risk_prob} and~\eqref{eq:expected_risk_multivariate} using gradient descent techniques. %\JL{Be more specific. Which optimizer and what hparams?}
Depending on the current state and data set, different hyperparameters perform better.
As a result, we perform extensive hyperparameter tuning every time we need to solve the optimization problem. Here, we sweep over gradient descent with momentum and Adam with learning rates between $0.005$ to $500$. 



We initialize each problem with $\bq_t$ equal to the baseline regression solution and $\bq_{t + s} = \bq_t / (s + 1)$ for all $1 \leq s \leq T - t$. That is, we set the initial value for future collection amounts to be fractions of the initial value of the immediate amount of data to collect. We identified this initialization by manually inspecting the solutions found by LOC, consequently it improves the conditioning of the loss landscape relative to other random initialization schemes.




==> How Much More Data Should I Get for ArXiv/sections/app_multivariate.tex <==
%\clearpage
\section{Optimal Data Collection with Multiple Sources}
\label{sec:app_multivariate}








The multi-variate data collection problem considers multiple sources delivering different types of data required to train a model. 
Consider $K$ data sets with $q^1, \dots, q^K$ points in each, respectively. 
Rather than collecting up to $q_t$ data points in each round, we optimize a vector $\bq_t \in \field{R}^K_+$ where each element $q^k_t$ refers to how much data we need from the $k$-th source.
Furthermore, the minimum data requirement is now a vector $\bD^*$. 


This problem can be solved using the same general approach outlined in Algorithm~\ref{alg:data_collection}, but with two changes.
First, we require a multi-variate version of the PDF and CDF of $\bD^*$. This necessitates new neural scaling law regression models for dealing with multiple data sources.
Second, we modify the optimization problem from Appendix~\ref{sec:app_opt} to accommodate decision vectors.
We highlight the above two steps in this section.





\subsection{A General Multi-variate Neural Scaling Law}




In order to construct a PDF and CDF in the multi-variate setting, we follow the same general steps as in Algorithm~\ref{alg:data_collection}.
%we follow the same general approach summarized in Section~\ref{sec:optimization_framework_learning} and Appendix~\ref{sec:app_opt}. 
We first collect a data set of performance statistics $\set{R} := \{ (\bq_r, V(\dataset^1_{q^1_r}, \dataset^2_{q^2_r}, \cdots, \dataset^K_{q^K_r} ) \}_{r=1}^R$ as before.
We then use bootstrap resamples of this data set to fit parameters $\btheta^*$ to a regression model $\hat{v}(q^1, \dots, q^K; \btheta)$ and then solve for 
%
\begin{align*}
    \hat{\bq} := \argmin_{\bq} \{ \bc^\tpose \bq \;|\; \hat{v}(q^1, \dots, q^K; \btheta^*) \geq V^* \}.
\end{align*}
%
Finally, we fit a density estimation model over our data set of $\hat{\bq}$. 


The key challenge to this approach however is in designing a multi-variate regression function.
To the best of our knowledge, the neural scaling law literature has not explored general power law models that can accommodate $K$ different types of data for arbitrary tasks.




We propose an easy-to-implement baseline regression model by adding the contributions of each data set being used.  Then, our additive regression model is
%
\begin{align*}
    \hat{v}(q^1, \dots, q^K; \btheta) := \sum_{k=1}^K \hat{v}_k(q^k; \btheta_k)
\end{align*}
%
where $\hat{v}_k(q_k; \btheta_k)$ can be any single-variate regression model for estimating score. For instance, consider $K=2$ data types with power law regression models for each data type. Our multi-variate regression model becomes
%
\begin{align*}
    \hat{v}(q^1, q^2; \btheta) = \theta_{1,0} (q^1)^{\theta_{1, 1}} + \theta_{2,0} (q^2)^{\theta_{2, 1}} + \theta_3.
\end{align*}
%
We may also incorporate other base models in the same way, such as the logarithmic or arctan functions introduced in~\citet{mahmood2022howmuch}.


The benefit of this additive regression model is that we can easily fit it via least squares minimization using a regression data set $\set{R} := \{ ( q^1_r, q^2_r, V(\dataset^1_{q^1_r}, \dataset^2_{q^2_r}) \}_{r=1}^R$. 
Furthermore, additive models are simple and offer interpretable explanations on the contributions of each data type to performance by assuming that each data set has an independent effect. 
Finally, additive models are common in many other tasks, such as when estimating the valuation of specific data points~\citep{ghorbani2019data}. 


We remark that some recent research has explored neural scaling laws for specific tasks with multiple data types.
For instance,~%multi-variate power laws have been studied in some limited respects.
\citet{mikami2021scaling} explore a $K=2$ power law for transfer learning from synthetic to real domains, where they use a multiplicative component that captures an interaction between real and synthetic data sets. 
Because scaling laws in multi-variate settings remain an open area of study, if there exist specific structural regression functions for a given application with different types of data, then such functions should be used in place of the additive model. 
Moreover, our downstream optimization model operates independently of the regression model, as long as the regression model can be re-trained with bootstrap samples in order to facilitate density estimation.




\subsection{The Optimization Problem with Multiple Decisions}


Just as in the single-variate case, problem~\eqref{eq:expected_risk_multivariate} has a differential objective function but a series of lower bound constraints. We can use the same approach highlighted in Appendix~\ref{sec:app_opt} to reformulate this problem and remove the constraints. We summarize this reformulation below.


For each $t$, let $\bd_t = \bq_t - \bq_{t-1}$ be the additional data collected in each round. Then, we recursively re-define $\bq_t = \bq_0 + \sum_{r=1}^t \bd_r$ and re-write the problem to
%
\begin{align*}
    \min_{\bd_1, \cdots \bd_T} \quad & \bc^\tpose \sum_{t=1}^T \bd_t \left( 1 - F\left(\bq_0 + \sum_{r=1}^{t-1} \bd_r \right) \right) + P \left( 1 - F\left(\bq_0 + \sum_{r=1}^T \bd_r\right) \right) \\ 
    \st\; \quad & \bd_1, \dots, \bd_T \geq 0.
\end{align*}
%
The above problem can now be solved using off-the-shelf gradient descent.




==> How Much More Data Should I Get for ArXiv/sections/app_notation.tex <==
\section{Table of Notation}
\label{sec:app_notation}



\begin{table}[!h]
    \centering
    \def\arraystretch{1.5}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c l}
        \toprule
        $T \in \mathbb{N}$ & Total number of rounds of collection.\\
        $V^* \in \mathbb{R}$ & Target performance.\\
        $P \in \mathbb{N}$ & Penalty for failing to reach target performance.\\
        $c \in \mathbb{N}$ & Cost of per-item collection.\\
        $q_t \in \mathbb{N}, \: t \in \{0,\ldots,T\}$ & Number of data points in round $t$.\\
        $\set{D}_q$ & Data set of size $q$.\\
        $V(\set{D})$ & Valuation of model trained on data set $\set{D}$.\\
        $V_q := V(\set{D}_q)$ & Short-hand notation for model valuation.\\
        $D^* := \argmin_q \left\{q \;|\; V_q \geq V^* \right\}$ & The minimum data requirement.\\
        $F(q) = P(D^* < q)$ & The CDF of the minimum data requirement.\\
        $f(q) = dF(q)/dq$ & The PDF of the minimum data requirement.\\
        $L(q_1,\ldots,q_T;D^*)$ & The stochastic objective function for data collection.\\
        $d_t \geq 0$ & Amount of data to collect in round $t$.\\
        $\set{R} := \left\{ (rq_t / R, V(\dataset_{rq_t/R})) \right\}_{r=1}^R $ & The regression set representing the learning curve of a given model and data set.\\
        $K \in \mathbb{N}$ & Number of data sources in multi-source setting.\\
        $\mathbf{q}_t \in \mathbb{N}^K$ & Vector containing number of data points per-source in round $t$.\\
        $\mathbf{c} \in \mathbb{N}^K$ & Vector of per-source costs.\\
        
        \bottomrule
    \end{tabular}
    }
    \caption{Table of notation used throughout paper.}
    \label{tab:notation}
\end{table}

==> How Much More Data Should I Get for ArXiv/sections/app_optimal_control.tex <==
\subsection{Optimal control framework}

In this section we introduce an optimal control perspective on our optimal data collection problem.

We define the state to be $q_t$, the amount of data that has been collected at time $t$. Within each round, a control $d_t \geq 0$ is chosen that corresponds to collecting $d_t$ new data points. At the end of each round, we pay a cost equal to $c d_t$ for some $c > 0$. We repeat this process for $T$ rounds and then we evaluate our model by computing $V_{q_T}$ and paying a penalty $P > 0$ if $V_{q_T} < V^*$. This describes an optimal control problem written as follows,
\begin{equation}
    \min_{d_0, \dots, d_{T-1}} \; \sum_{t=0}^{T-1}c d_t + P \Ind \{ V(\dataset_{q_T}) < V^* \} \quad\;\; \st \; d_t \geq 0,\textrm{ and }\:q_{t+1} = q_t + d_t.
\end{equation}
This is a stochastic control problem whose expected loss is written,
\begin{equation}
    \min_{d_0, \dots, d_{T-1}} \; \sum_{t=0}^{T-1}c d_t + P (1 - F(q_T)) \quad\;\; \st \; d_t \geq 0, \:\forall t.
\end{equation}
We can derive the control Hamiltonian,
\begin{equation}
    H = c d_t + \lambda_{t+1} d_t,
\end{equation}
where $\lambda_t$ is the costate. Pontryagin's maximum principle states that,
\begin{align*}
    q_{t+1} - q_t &= d_t,\\
    \lambda_{t+1} - \lambda_t &= 0,\\
    \lambda_T &= -Pf(q_T),\\
    d^*_t &= \arg\min_{d_t} H(q_t, d_t, \lambda_{t+1}).
\end{align*}
Solving the last equation gives us $\lambda_{t+1} = -c$, and using the fact that $\lambda_t$ is constant we recover $f(q_T) = c/P$. \JL{If you take the same $P^*$ as used in Theorem 1, you recover the same optimal choice for $q_T$. Further, you could add in $(1-F(q_{t+1}))$ to the per-round cost function to match our objective. But I'm not sure if this is necessary. I feel that we should recover an optimal policy if we correctly handle uncertainty in quantifying the distribution.}

==> How Much More Data Should I Get for ArXiv/sections/app_optimization_algo.tex <==
%\clearpage
\section{Learn-Optimize-Collect}
\label{sec:app_opt}





Algorithm~\ref{alg:data_collection} summarizes the complete workflow of LOC within the data collection problem. 
Given a target score $V^*$, we collect data until we have met the target or until $T$ rounds have passed. 
In this section, we first expand our complete LOC algorithm. 
We then provide further details on the regression procedure used to estimate the data requirement distributions. 
Finally, we introduce a more practical reformulation of our optimization problem~\eqref{eq:expected_risk_prob}, which is what we later use in our numerical experiments.



\subsection{Details on the Learning and Optimizing Approach}


Our approach for determining how much data to collect consists of three steps. 
The first step is to collect performance statistics by measuring the training dynamics of the current data set $\dataset_{q_t}$. Here, we sample subsets of the current data set, train our model on the subset, and evaluate the score. We repeat this process for up to $R$ subsets, where $R$ denotes the size of our performance statistics regression data set $\set{R}$.



The second step is to model the data requirement distribution $D^*$. We perform this by creating bootstrap samples from $\set{R}$, and then fitting a regression model $\hat{v}(q;\btheta)$ that can estimate the model score as a function of data set size. We then invert this regression function by solving for the minimum $\hat{q}$ for which the model will predict that we have exceeded the target performance. We repeat this process to obtain $B$ bootstrap estimates of $D^*$. We can then fit any density estimation model to approximate a probability density and a cumulative density function. In this paper, we focus on Kernel Density Estimation (KDE) and Gaussian Mixture models since such models can be easily fit and provide functional forms of the PDF. 



Finally in the third step, we solve our optimization problem~\eqref{eq:expected_risk_prob} via gradient descent. This problem yields the optimal data set sizes $q_1^*, \dots, q_T^*$ that we should have at the end of each round. Furthermore, if we are in the $t$-th round for $t > 1$, we freeze the values for $q_1, \dots, q_{t-1}$ to the data set sizes that we have observed in the previous rounds. 
Upon solving this problem, we then collect data until we have $q_t$ samples, and then re-train our model to evaluate our current state.









%\iffalse
%\rrm{I commented out the algorithm, but we can bring it back later if we want. I feel we should keep only one of the algorithm or Fig 2?}
%\begin{figure}[t!]
\begin{algorithm}[t!]
\footnotesize
\caption{Learn-Optimize-Collect (LOC)}\label{alg:data_collection}
\begin{algorithmic}[1]
\State \textbf{Input:}  Initial data set $\dataset_{q_0}$, Sampling distribution $p(z)$, Score function $V(\dataset)$, Target score $V^*$, Maximum rounds $T$, Cost $c$, Penalty $P$, Regression model $\hv(q;\btheta)$, Regression set size $R$, Density Estimation model $f(q)$, Number of bootstrap samples $B$. 
%
\State Initialize round $t = 0$, loss $L = 0$
\Repeat
    \Procedure{Collect Performance Statistics}{}
    \State Initialize $\set{R} = \emptyset$, $\dataset_{0} = \emptyset$
    \For{$r \in \{1, \dots, R\}$}
        \State Sub-sample $\dataset_{q_tr/R} \subset \dataset_{q_t}$ by augmenting to $\dataset_{q_t(r-1)/R}$
        %\JL{Not obvious it's growing sequentially}
        \State Evaluate $V(\dataset_{q_tr/R})$ and update $\set{R} \gets \set{R} \cup \{ ( q_tr/R , V(\dataset_{q_tr/R}) \}$
    \EndFor
    \EndProcedure
    \Procedure{Estimate Data Requirement Distribution}{}
    \State Initialize $\set{Q} = \emptyset$
    \For{$b \in \{1, \dots, B\}$}
        \State Create bootstrap $\set{R}_b$ by sub-sampling with replacement from $\set{R}$
        \State Fit regression model
            $\btheta^* = \argmin_{\btheta} \sum_{(q, v) \in \set{R}_b} \left(v - \hat{v}(q; \btheta)\right)^2$
        %\begin{align*}
        %    \btheta^* = \argmin_{\btheta} \sum_{(q, v) \in \set{R}_b} \left(v - \hat{v}(q; \btheta)\right)^2
        %\end{align*}
        \State Estimate data requirement
            $\hat{q}_b = \argmin_{q} \left\{ q \;|\; \hat{v}(q; \btheta^*) \geq V^* \right\}$
        %
        %\begin{align*}
        %    \hat{q} = \argmin_{q} q \;\; \st \; \hat{v}(q; \btheta^*) \geq V^*
        %\end{align*}
        \State Update $\set{Q} \gets \set{Q} \cup \{ \hat{q}_b \}$
    \EndFor
    \State Fit Density Estimation model $f(q)$ using the empirical distribution $\set{Q}$ and let $F(q) = \int_{0}^q f(q)dq$
    \EndProcedure
    \Procedure{Collect Data}{}
        \State Solve problem~\eqref{eq:expected_risk_prob} using Density Estimation models $f(q)$ and $F(q)$ to obtain $q^*_1, \dots, q^*_T$.
        \State Sample $\hat\dataset \sim p(z)$ until $|\hat\dataset| = q_{t} - q_{t-1}$
        \State Update loss $L \gets L + c (q_{t} - q_{t-1}) $
        \State Update $\dataset_{q_{t}} = \dataset_{q_{t-1}} \cup \hat\dataset$
    \EndProcedure
    \State Evaluate $V(\dataset_{q_t})$ and update $t \gets t + 1$ 
\Until{$V(\dataset_{q_t}) \geq V^*$ or $t = T$}
\If{$V(\dataset_{q_t}) < V^*$}
    \State Update loss $L \gets L + P$
\EndIf
\State \textbf{Output:} Final collected data set $\dataset_{q_t}$, loss $L$
\end{algorithmic}
\end{algorithm}
%\end{figure}






\subsection{Regression Model for $D^*$}



To estimate the data requirement, we build a regression model of the learning curve and then invert this curve. 
The classical learning curve literature proposes using structured functions to regress on the learning curve.
For example with neural scaling laws, the most common function is a power law model $\hat{v}(q;\btheta) := \theta_0 q^{\theta_1} + \theta_2$ where $\btheta := \{ \theta_0, \theta_1, \theta_2 \}$~\citep{hestness2017deep, viering2021shape, sun2017revisiting, rosenfeld2019constructive, bahri2021explaining, bisla2021theoretical, zhai2021scaling, hoiem2021learning, mahmood2022howmuch}. 
As a result, the main experiments of our paper use this model.




We fit each regression function by minimizing a least squares problem using the Levenberg-Marquardt algorithm as implemented by Scipy~\cite{more1978levenberg, 2020SciPy-NMeth}. The parameters for each function are initialized to either $1$ or $0$ depending on if they are product or bias terms. To further help fit the data, we use weighted least squares where each subsequent point is weighted twice as much as the previous point. This ensures that our regression model is tuned to better fit the curve for larger $q$. 










\subsection{Alternate Re-formulation of Problem~\eqref{eq:expected_risk_prob}}



Although problem~\eqref{eq:expected_risk_prob} has a differentiable objective function, it includes a set of lower bound constraints, meaning that a vanilla gradient descent algorithm may not immediately apply.
A naive solution algorithm may be to use projected gradient descent. 
Instead, we show that the problem can be reformulated to remove these constraints.


For each $t$, let $d_t = q_t - q_{t-1}$ denote the additional amount of data collected in each round. Note that we can recursively re-define $q_t = q_0 + \sum_{r=1}^t d_r$. Furthermore, the ordering inequality constraints can all be re-written to non-negativity constraints $d_t \geq 0$. We now re-write problem~\eqref{eq:expected_risk_prob} using these new variables:
%
\begin{align*}
    \min_{d_1, \cdots d_T} \quad & c \sum_{t=1}^T d_t \left( 1 - F\left(q_0 + \sum_{r=1}^{t-1} d_r \right) \right) + P \left( 1 - F\left(q_0 + \sum_{r=1}^T d_r\right) \right) \\ 
    \st\; \quad & d_1, \dots, d_T \geq 0.
\end{align*}
%
The objective in the above formulation remains differentiable. Moreover, the non-negativity constraints can be removed by re-writing $d_t \gets \mathrm{softplus}(d_t)$ for all $t$. As a result, we can solve this problem by using an off-the-shelf gradient descent algorithm. 
Finally we note that in our experiments, we implemented a projected gradient descent based on~\eqref{eq:expected_risk_prob} and the above gradient descent algorithm. We found that the above streamlined approach to generate slightly better final solutions.







==> How Much More Data Should I Get for ArXiv/sections/app_proofs.tex <==
%\clearpage
\section{Details on the Main Theory}
\label{sec:app_math_properties_one_d}

In this section, we explore mathematical properties and challenges of the optimal data collection problem. In Section~\ref{sec:app_mdp_alternatives}, we discuss the drawbacks of alternative approaches to our modeling framework. Then in Section~\ref{sec:app_proofs}, we prove our main theorem demonstrating an analytic solution in the single-round problem.





\subsection{Markov Decision Process Alternatives}
\label{sec:app_mdp_alternatives}



The data collection problem requires sequential decision-making in terms of collecting additional data in each round. A natural modeling approach for such problems is via Markov Decision Processes (MDPs).
However, MDP techniques are challenging for this problem due to (i) the unobservability of the state, and (ii) an infinite state space. 
That is, until we have collected enough data to meet the target, we do not know how much data is the minimum, which can furthermore be arbitrarily large. 
Here, we sketch a potential alternative MDP framework and highlight the core challenge.






Our sequential decision-making problem
%is governed by the minimum data requirement $D^*$, which is an unobserved state variable. As a result, this problem 
can be written as a Partially Observable Markov Decision Process (POMDP)~\citep{puterman2014markov, bertsekas2012dynamic}. Furthermore, because this state variable is constant throughout the collection problem, we can write it as an EK `Learning-and-Doing' model~\citep{easley1988controlling}. Such POMDPs are defined by the tuple $(\Theta, \set{A}, \set{S}, p, r_t)$, 
where the state space characterizes the data requirement $D^* \in \Theta := \field{R}_+$, the action space characterizes the additional data collected $d_t := (q_t - q_{t-1}) \in \set{A} := \field{R}_+$, and the observation set $\set{S} := \{0,1\}$ characterizes a binary variable $\Ind \{ V(\dataset_{q_t}) \geq V^* \} = \Ind \{ q_t \geq D^* \}$. 
Furthermore, $p( \cdot | D^*, d_t)$ is the observation transition probability and $r_t(\cdot)$ is the reward function where $r_t(q_t, q_{t-1}, D^*) := -c (q_t -  q_{t-1})$ for $t \leq T$ and $r_{T+1}(q_t, q_{t-1}, D^*) := -P \Ind \{ q_T < D^* \}$.




Because the state variable is unobserved, POMDPs are typically solved by using a belief distribution of the state variable to average the reward in the value function.
When both the state and the action space of a POMDP are finite,~\citet{smallwood1973optimal} show that this value function is piecewise-linear and can be solved by exact methods, albeit under a curse of dimensionality with respect to these spaces.
Unfortunately, for a general POMDP with an infinite state and action space, 
these methods do not apply and we most often resort to approximation techniques~\citep{zhao2021active}. 
Moreover in our case, approximations based on discretizing the state and action space fall prey to the curse of dimensionality.




Alternatively, we may naively consider applying reinforcement learning.
However, note that real-world data collection tasks do not contain the requisite sizes of learning data or generalizable simulation mechanisms that are staples in reinforcement learning techniques. 
These challenges, coupled with the goal of delivering practical managerial guidelines for data collection operations,
motivate us to explore easy-to-implement techniques for optimizing data collection.






























\subsection{Proof of Theorem~\ref{thm:t1_has_analytic_sol}}
\label{sec:app_proofs}











Our main theorem states that the one-round problem has an analytic solution. 
However, the proof requires several auxiliary results.
For clarity, we first reproduce the theorem.


\noindent\textbf{Theorem 1 (Repeated).}
%\begin{thm}%\label{thm:t1_has_analytic_sol}
\emph{
    Consider the one-round problem
    %
    \begin{align*}
        \min_{q_1} \; c(q_1 - q_0) + P(1 - F(q_1)) \quad\quad \st \; q_0 \leq q_1
    \end{align*}
    %
    Assume $F(q)$ is strictly increasing and continuous. For any $\epsilon$ such that $F(q_0) < 1 - \epsilon$, let
    $P := c / f ( F^{-1}(1 - \epsilon) )$. The optimal solution to the corresponding problem~\eqref{eq:expected_risk_prob_one_round} is $q_1^* = F^{-1}(1 - \epsilon)$. Furthermore, the optimal solution satisfies $F(q_1^*) = 1 - \epsilon$.
%\end{thm}
}

The assumption of a strictly increasing and continuous cumulative density function is needed to ensure that the data requirement distribution has a well-defined quantile function $F^{-1}(p) := \inf_{q} \{ q \;|\; F(q) \geq p \}$, where the optimal solution for any $p \in (0, 1)$ is unique.



The proof for Theorem~\ref{thm:t1_has_analytic_sol} relies on equating the one-round optimization problem to the following constrained optimization problem:
%
\begin{align}\label{eq:constrained_expected_risk}
    \min_{q_1} \; c(q_1 - q_0) \qquad \st \; F(q_1) \geq 1 -\epsilon \;, \;\; q_0 \leq q_1
\end{align}
%
where $\epsilon > 0$ is a pre-determined parameter. This above problem~\eqref{eq:constrained_expected_risk} is solving for the least amount of additional data to collect such that with probability at least $1 - \epsilon$, we collect above the minimum data requirement.
We first characterize the properties of problem~\eqref{eq:constrained_expected_risk}.
%
\begin{lem}\label{lem:constrained_expected_risk_is_convex}
    Problem~\eqref{eq:constrained_expected_risk} is a convex optimization problem.
\end{lem}
%
\begin{proof}
    We only need to prove that the set $\{ q_1 \;|\; F(q_1) \geq 1 - \epsilon \}$ is a convex set, since the objective and remaining constraint are convex. 
    Since $F(q)$ is a monotonically non-decreasing function in $q$, for any $\theta \in [0, 1]$ and $q < \hat{q}$ that satisfy the CDF constraint, we have
    %
    \begin{align*}
        F(\theta q + (1-\theta) \hat{q}) \geq F(q) \geq 1 - \epsilon.
    \end{align*}
    %
    Because the convex combination of any two points is in the set, the set must be convex.
\end{proof}
%
\begin{lem}\label{lem:constrained_expected_risk_has_opt}
    The optimal solution to problem~\eqref{eq:constrained_expected_risk} is
    %
    \begin{align*}
        q^* = 
        \begin{cases}
            F^{-1}(1 - \epsilon), & \text{ if } F(q) < 1 - \epsilon \\
            q_0 & \text{ otherwise}
        \end{cases}
    \end{align*}    
\end{lem}
%
\begin{proof}
    First consider the case where $F(q_0) \geq 1 - \epsilon$. Then, $q_0$ is a feasible solution to problem~\eqref{eq:constrained_expected_risk}. Furthermore due to the second constraint, any $q < q_0$ is infeasible. Since $q_0$ minimizes the objective, it is optimal.
    
    Next consider the case where $F(q_0) < 1 - \epsilon$. Then, let $q_1 = F^{-1}(1 - \epsilon) = \inf \{ q \;|\; F(q) \geq 1 - \epsilon \}$ be the smallest solution that satisfies the CDF constraint. By the monotonicity of $F(q)$, it follows that $q_1 > q_0$. Therefore, this solution minimizes the objective.
\end{proof}


We are now ready to prove Theorem~\ref{thm:t1_has_analytic_sol}.


\begin{proof}[Proof of Theorem~\ref{thm:t1_has_analytic_sol}.]
    %The proof follows similar 
    We prove this result by first developing two different characterizations of the optimal solution set of problem \eqref{eq:expected_risk_prob_one_round} and then applying their equivalence.
    
    First note that problem \eqref{eq:expected_risk_prob_one_round} is an optimization problem with one variable $q_1$ over a constrained domain $[q_0, \infty)$. Furthermore, the objective function is continuous everywhere, meaning that there are two possible scenarios:
    %
    \begin{itemize}
        \item $q_1^*$ satisfies $f(q_1) = c/P$. 
        
        \item $q_1^* := q_0$ and the optimal value is $P(1 - F(q_0))$.
        %\item $q_1^* \rightarrow + \infty$ and the optimal value is unbounded.
    \end{itemize}
    %
    The first scenario is obtained by taking the derivative of the objective function and setting it to $0$.
    The second scenario comes from the boundary condition. Moreover, note that the objective is unbounded as $q_1 \rightarrow +\infty$ meaning the above scenario is the only boundary condition that we need to consider. 
    
    
    Next, note that problem \eqref{eq:expected_risk_prob_one_round} is equivalent to the following optimization problem
    %
    \begin{align} \label{eq:expected_risk_prob_one_round_recast}
    \begin{split}
        \min_{q_1, \epsilon} \quad & c (q_1 - q_0) + P \epsilon \\
        \st \quad   & \epsilon \geq 1 - F(q_1) \\
                    & q_1 \geq q_0
    \end{split}
    \end{align}
    %
    
    \begin{align*}
        \min_\epsilon c(F^{-1}(1- \epsilon) - q_0) + P\epsilon \qquad \st \epsilon \geq 1 - F(q_0)
    \end{align*}
    
    For any fixed $\epsilon$, problem \eqref{eq:expected_risk_prob_one_round_recast} is equivalent to problem \eqref{eq:constrained_expected_risk}, and therefore by Lemma \ref{lem:constrained_expected_risk_is_convex}, the problem is convex optimization problem. 
    
    We can optimize problem \eqref{eq:expected_risk_prob_one_round_recast} by breaking into two cases. 
    First, for any fixed $\epsilon \geq 1 - F(q_0)$, setting $q_1^*(\epsilon) = 0$ attains a feasible solution and mnimizes the objective to $P\epsilon$. 
    
    Second, for any fixed $\epsilon \leq 1 - F(q_0)$,  Lemma \ref{lem:constrained_expected_risk_has_opt} states that $q_1^*(\epsilon) = F^{-1}(1 - \epsilon)$ is a corresponding optimal solution and the objective function reduces to
    %
    \begin{align*}
        c\left( F^{-1}( 1 - \epsilon ) - q_0 \right) + P \epsilon.
    \end{align*}
    %
    Moreover, from the original formulation \eqref{eq:expected_risk_prob_one_round}, we can substitute $q_1^*(\epsilon)$ and obtain $f(F^{-1}(1 - \epsilon) = c / P$.
    
    
    Finally, problem \eqref{eq:expected_risk_prob_one_round_recast} is optimized via the second case if and only if there exists a feasible $\epsilon \leq 1 - F(q_0)$ that satisfies
    %
    \begin{align*}
        c\left( F^{-1}( 1 - \epsilon ) - q_0 \right) + P \epsilon \leq P (1 - F(q_0)).
    \end{align*}
    %    
    We can rewrite this condition as follows. Let $q_1 > q_0$ and assume that \eqref{eq:expected_risk_prob_one_round_required_condition} holds. Then, 
    %
    \begin{align*}
        & c (q_1 - q_0) \leq P F(q_1) - P F(q_0) \\
        \Rightarrow\quad & c (q_1 - q_0) - P F(q_1) \leq  - P F(q_0) \\
        \Rightarrow\quad & c (q_1 - q_0) + P ( 1 -  F(q_1)) \leq P (1 - F(q_0)).
    \end{align*}
    %
    Let $\epsilon = 1 - F(q_1)$. Since $F(q_1) \geq F(q_0)$, we have $\epsilon \leq 1 - F(q_0)$, meaning that there is a feasible $q_1 > q_0$ to problem \eqref{eq:expected_risk_prob_one_round_recast} with lower objective function value than $q_0$. 
    Thus, assumption \eqref{eq:expected_risk_prob_one_round_required_condition} guarantees that problem \eqref{eq:expected_risk_prob_one_round_recast} has an optimal solution $q_1^* = F^{-1}(1 - \epsilon^*)$ where $\epsilon^*$ must satisfy $f(F^{-1}(1 - \epsilon^*) = c / P$. 
    Conversely, if \eqref{eq:expected_risk_prob_one_round_required_condition} is not satisfiable for any $q_1 > q_0$, then we can use the same steps to show that $q_1^* = q_0$ is an optimal solution to the problem.
\end{proof}



==> How Much More Data Should I Get for ArXiv/sections/conclusion.tex <==
\section{Discussion}
\label{sec:conclusion}





We develop a rigorous framework for optimizing data collection workflows in machine learning applications, by introducing an optimal data collection problem that captures the uncertainty in estimating data requirements. %; our problem can be solved with gradient descent techniques. 
We generalize this problem to more realistic settings where multiple data sources incur different collection costs. 
We validate our solution algorithm, LOC, on six data sets covering classification, segmentation, and detection tasks to show that we consistently meet pre-determined performance metrics regardless of costs and time horizons.




Our approach relies on estimating the CDF and PDF of the minimum data requirement, which is a challenging problem, especially with multiple data sources. 
Nonetheless, LOC can be deployed on top of future advances in estimating neural scaling laws.
Further, we allow practitioners to input problem-specific costs and penalties, but these quantities may not always be readily available.
We provide some theoretical insight into parameter selection and show that LOC is robust to these parameters.
Finally, our empirical analysis focuses on computer vision, but we expect our approach to be viable in other domains governed by scaling laws.



Improving data collection practices yields potentially positive and negative societal impacts. 
LOC reduces the collection of extraneous data, which can, in turn, reduce the environmental costs of training models.
On the other hand, equitable data collection should also be considered in real-world data collection practices that involve humans. 
We envision a potential future work to incorporate privacy and fairness constraints to prevent over- or under-sampling of protected groups.
Finally, our method is guided by a score function on a held-out validation set. Biases in this set may be exacerbated when optimizing data collection to meet target performance.









There is a folklore observation that over $80\%$ of industry machine learning projects fail to reach production, often due to insufficient, noisy, or inappropriate data~\citep{van_der_meulen_mccall_2018, venturebeat_2019}. 
Our experiments verify this by showing that na\"{i}vely estimating data requirements will often yield failures to meet target performances. 
We believe that robust data collection policies obtained via LOC can reduce failures while further guiding practitioners on how to manage both costs and time.






==> How Much More Data Should I Get for ArXiv/sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}





When deploying a deep learning model in an industrial application, designers often mandate that the model must meet a pre-determined baseline performance, such as a target metric over a validation data set. 
For example, an object detector may require a certain minimum mean average precision before being deployed in a safety-critical setting. 
One of the most effective ways of meeting target performances is by collecting more training data for a given model. 



Determining how much data is needed to meet performance targets can impact costs and development delays.
%in deep learning workflows. 
Overestimating the data requirement incurs excess costs from collection, cleaning, and annotation. 
For instance, annotating segmentation masks for a driving data set takes between $15$ to $40$ seconds per object. For $100{,}000$ images the annotation could require between $170$ and $460$ days-equivalent of time~\citep{acuna2018efficient, mahmood2022howmuch}.
On the other hand, collecting too little data may incur future costs and workflow delays from having to collect more later. 
For example, in medical imaging applications, this means further clinical data acquisition rounds
% processes
that require expensive clinician time. 
In the worst case, designers may even realize that a project is infeasible only after collecting insufficient data. 






The growing literature on sample complexity in machine learning has identified neural scaling laws that scale model performance with data set sizes according to power laws
\citep{frey1999modeling, gu2001modelling, hestness2017deep, rosenfeld2019constructive, kaplan2020scaling, hoiem2021learning, bahri2021explaining, bisla2021theoretical}.
For instance,~\citet{rosenfeld2019constructive} fit power law functions on the performance statistics of small data sets to extrapolate the learning curve with more data.
In contrast,~\citet{mahmood2022howmuch} consider estimating data requirements and show that even 
small errors in a power law model of the learning curve can translate to massively over- or underestimating how much data is needed.
Beyond this, different data sources have different costs and scale differently with performance~\citep{mikami2021scaling,acuna2021f,Prakash_2021_ICCV,acuna2022domain}.
For example, although unlabeled data may be easier to collect than labeled data, some semi-supervised learning tasks may need an order of magnitude more unlabeled data to match the performance of a small labeled set. 
Thus, collecting more data based only on estimation will fail to capture uncertainty and collection costs. 




In this paper, we propose a new paradigm for modeling the data collection workflow as an \emph{optimal data collection problem}. Here, a designer must minimize the cost of collecting enough data to obtain a model capable of a desired performance score.
%In this problem, a designer collects data to obtain a model capable of a target performance score.
They have multiple collection rounds, where after each round, they re-evaluate the model and decide how much more data to order.
The data has per-sample costs and moreover, the designer pays a penalty if they fail to meet the target score within a finite horizon. 
Using this formal framework, we develop an optimization approach for minimizing the expected future collection costs and show that this problem can be optimized in each collection round via gradient descent. 
Furthermore, our optimization problem immediately generalizes to decisions over multiple data sources (e.g., unlabeled, long-tail, cross-domain, synthetic) that have different costs and impacts on performance. 
Finally, we demonstrate the value of optimization over na\"{i}vely estimating data set requirements (e.g.,~\citep{mahmood2022howmuch}) for several machine learning tasks and data sets. %; in nearly every case, we significantly reduce the chances of failing to meet the performance target.







Our contributions are as follows.
(1) We propose the optimal data collection problem in machine learning, which formalizes data collection workflows.
(2) We introduce Learn-Optimize-Collect (LOC), a learning-and-optimizing framework that minimizes future collection costs, can be solved via gradient descent, and has analytic solutions in some settings. %\SF{introduce LOC?}
(3) We generalize the data collection problem and LOC to a multi-variate setting where different types of data have different costs. To the best of our knowledge, this is the first exploration of data collection with general multiple data sets in machine learning, covering for example, semi-supervised and long-tail learning. 
(4) We perform experiments over classification, segmentation, and detection tasks to show, on average, approximately a $2\times$ reduction in the chances of failing to meet performance targets, versus estimation baselines. % rates the power of optimization over naive estimation of data requirements.








==> How Much More Data Should I Get for ArXiv/sections/multivariate.tex <==
% \section{The Multi-variate Extension with Different Data Sets}

%\newpage 

\section{The Multi-variate LOC: Collecting Data from Multiple Sources}
\label{sec:multivariate}




So far, we have assumed that a designer only chooses how much data to collect and must pay a fixed per-sample collection cost. 
We now explore the multi-variate extension of the data collection problem where there are different types of data with different costs. 
For example, consider long-tail learning where samples for some rare classes are harder to obtain and thus, more expensive~\citep{haixiang2017learning}, semi-supervised learning where labeling data may cost more than collecting unlabeled data~\citep{van2020survey},
%we may collect labeled data at a higher cost than unlabeled data~\citep{van2020survey}, 
or domain adaptation where a source data set is easier to obtain than a target set~\citep{ben2010theory}. 
In this section, we highlight our main formulation and defer the complete multi-variate LOC to Appendix~\ref{sec:app_multivariate}.


Consider $K \in \field{N}$ data sources (e.g., $K=2$ with labeled and unlabeled) and for each $k \in \{1, \dots, K\}$, let $z^k \sim p_k(z^k)$ be data drawn from their distribution. We train a model with a data set $\dataset := \cup_{k=1}^K \dataset^k$ where each $\dataset^k$ contains points of the $k$-th source. 
The performance or score function of our model is $V(\dataset^1, \dots, \dataset^K)$. For each $k$, we initialize with $q_0^k$ points. Let $\bq_0 = (q^1_0, \dots, q^K_0)^\tpose$ denote the vector of data set sizes and let $\bc = (c^1, \dots, c^K)^\tpose$ denote costs (i.e., $c^k$ is the cost of collecting data from $p_k(z^k)$). 
Given a target $V^*$, penalty $P$, and $T$ rounds, we want to minimize the total cost of collection
%
\begin{equation*}
    \min_{\bq_1, \dots, \bq_T} \; \bc^\tpose \sum_{t=1}^T(\bq_t - \bq_{t-1}) + P \Ind \{ V(\dataset_{q_T^1}, \dots, \dataset_{q_T^K}) < V^* \} \quad\;\; \st \; \bq_0 \leq \bq_1 \leq \bq_2 \leq \cdots \leq \bq_T
\end{equation*}
%In order to solve this problem, 
We follow the same steps shown in Section~\ref{sec:optimization_framework} for this problem. First, the learning curve is now a stochastic process $\{ V_{\bq} \}_{\bq \in \field{Z}_+^K}$ indexed in $K$ dimensions. Next, the multi-variate analogue of the minimum data requirement in~\eqref{eq:min_dat_req} is the minimum cost amount of data needed to meet the target: % (we randomly pick a unique solution to break ties): 
%how much of each data type is required to meet the target score:
%
\begin{align*}
    \bD^* := \argmin_{\bq} \left\{ \bc^\tpose \bq \;|\; V_{\bq} \geq V^* \right\}
\end{align*}
%
We randomly pick a unique solution to break ties.
From Assumption~\ref{ass:cdf_pdf_exists}, $\bD^*$ is a random vector with a PDF $f(\bq)$ and a CDF $F(\bq) := \int^{\bq}_{\bzero} f(\bhq) d\bhq$. 
Finally, the multi-variate analogue of problem~\eqref{eq:expected_risk_prob} is 
%Finally, the multi-variate analogue of the stochastic problem~\eqref{eq:expected_risk_prob} is 
%
\begin{align}\label{eq:expected_risk_multivariate}
    \min_{\bq_1, \cdots, \bq_T} \; \bc^\tpose \sum_{t=1}^T (\bq_t - \bq_{t-1}) \left( 1 - F(\bq_{t-1}) \right) + P \left( 1 - F(\bq_T) \right) \; \st \; \bq_0 \leq \bq_1 \leq \cdots \leq \bq_T
\end{align}
%
The Multi-variate LOC requires multi-variate PDFs, which we can fit in the same way as discussed in Section~\ref{sec:optimization_framework_learning}. 
However, we now need multi-variate regression functions that can accommodate different types of data.
In Appendix~\ref{sec:app_multivariate}, we propose an additive family of power law regression functions that can handle an arbitrary number of $K$ sources. In our experiments, we also generalize the estimation approach of \citet{mahmood2022howmuch} to the multi-source setting for comparison.





==> How Much More Data Should I Get for ArXiv/sections/optimization_method.tex <==



\section{Learn-Optimize-Collect (LOC)}
\label{sec:optimization_framework}





%First, the data collection variables should be discrete $q_1, \dots, q_T \in \field{Z}_+$. However, because their values are on the order of thousands or greater, we relax the integrality requirement to optimize over continuous variables and afterwards round the solutions.

%\clearpage




Our solution approach, which we refer to as Learn-Optimize-Collect (LOC), minimizes the total collection cost while incorporating the uncertainty of estimating $D^*$. 
Although $D^*$ is a discrete random variable, it is realized typically on the order of thousands or greater. 
To simplify our problem and ensure differentiability, we assume that $D^*$ is continuous and has a well-defined density.
%
\begin{assumption}\label{ass:cdf_pdf_exists}
The random variable $D^*$ is absolutely continuous and has a cumulative density function (CDF) $F(q)$ and probability density function (PDF) $f(q) := dF(q)/dq$.
\end{assumption}
%
%Assumption~\ref{ass:cdf_pdf_exists} is necessary to allow our optimization problem to be differentiable. 
In Section~\ref{sec:optimization_framework_opt_problem}, we first develop an optimization model when given access to the CDF $f(q)$ and PDF $F(q)$. 
In Section~\ref{sec:optimization_framework_learning}, we estimate these distributions and combine them with the optimization model.
Finally in Section~\ref{sec:compare_vs_CVPR}, we delineate our optimization approach from prior regression methods.


%In Section~\ref{sec:optimization_framework_learning}, we propose estimating these distributions, before combining them with the optimization model. 



%We provide full details, including the complete Algorithm in Appendix~\ref{sec:app_opt}.




\iffalse
    In this section, we propose our solution approach, Learn-Optimize-Collect (LOC), for minimizing the total collection cost while incorporating the uncertainty of estimating $D^*$.
    %In this section, we propose an optimization framework for minimizing the total cost of collection while incorporating the uncertainty of estimating the data requirement $D^*$. 
    Our framework assumes that the stopping time of the learning curve stochastic process is a well-defined random variable.
    %
    \begin{assumption}\label{ass:cdf_pdf_exists}
    The random variable $D^*$ is measurable and has a cumulative density function (CDF) $F(q)$ and probability density function (PDF) $f(q) := dF(q)/dq$.
    \end{assumption}
    %
    In Section~\ref{sec:optimization_framework_opt_problem}, we first develop an optimization model when given access to the CDF $f(q)$ and PDF $F(q)$. 
    In Section~\ref{sec:optimization_framework_learning}, we propose estimating these distributions, before combining them with the optimization model. 
    %Combining these two steps completes our solution approach.
    %Finally in Section~\ref{sec:choosing parameters}, we 
    We provide full details, including the complete Algorithm in Appendix~\ref{sec:app_opt}.
\fi






\subsection{Optimization Model}
\label{sec:optimization_framework_opt_problem}





We propose an optimization problem that for any $t$, can simultaneously solve for the optimal amounts of data to collect $q_t, \dots, q_{T}$ in all future rounds. Consider $t=1$ 
and to develop intuition, suppose we know a priori the exact stopping time $D^*$. 
%In order to develop intuition, let us first suppose that we know a priori the exact stopping time $D^*$ 
Then, problem~\eqref{eq:formal_problem} can be re-written as
%
\begin{equation} \label{eq:original_prob}
    \min_{q_1, \cdots q_T} \; L(q_1, \dots, q_T; D^*)  \qquad\qquad \st \; q_0 \leq q_1 \leq \cdots \leq q_T
\end{equation}
%
where the objective function is defined recursively as follows
%
\begin{align*}
    L(q_1, \dots, q_T; D^*) &:= c (q_1 - q_0) + \Ind \{ q_1 < D^* \} \Big( c (q_2 - q_1) + \Ind \{ q_2 < D^* \} \Big( c (q_3 - q_2) \dots \\
        & \qquad \qquad \;\; \dots + \Ind \{ q_{T-1} < D^* \} \Big( c (q_T - q_{T-1}) + P \Ind \{q_T < D^*\} \Big)\cdots\Big)\Big) \\
        &= c \sum_{t=1}^T (q_t - q_{t-1}) \prod_{s=1}^{t-1} \Ind \{ q_s < D^* \}  + P \prod_{t=1}^T  \Ind \{ q_s < D^* \} \\
        &= c \sum_{t=1}^T (q_t - q_{t-1}) \Ind \{ q_{t-1} < D^* \}  + P \Ind \{ q_T < D^* \}.
\end{align*}
%
The objective differs slightly from \eqref{eq:formal_problem} due to the indicator terms, which ensure that once we collect enough data, we terminate the problem.
The second line follows from gathering the terms. The third line follows from observing that $q_1 \leq q_2 \leq \cdots \leq q_T$ are constrained.
%The second line follows from gathering the terms. The third line follows from observing that since $q_1 \leq q_2 \leq \cdots \leq q_T$ are constrained, the product of the indicators is equal to the maximum.


In practice, we do not know $D^*$ a priori since it is an unobserved random variable.
Instead, suppose we have access to the CDF $F(q)$. Then, we take the expectation over the objective $\field{E} [ L(q_1, \dots, q_T; D^*) ]$ to formulate a \emph{stochastic optimization problem} for determining how much data to collect:
%
\begin{equation} \label{eq:expected_risk_prob}
    \min_{q_1, \cdots q_T} \; c \sum_{t=1}^T (q_t - q_{t-1}) \left( 1 - F(q_{t-1}) \right) + P \left( 1 - F(q_T) \right) \quad \st \; q_0 \leq q_1 \leq \cdots \leq q_T.
\end{equation}
%
Note that the collection variables should be discrete $q_1, \dots, q_T \in \field{Z}_+$, but similar to the modeling of $D^*$, we relax the integrality requirement, optimize over continuous variables, and round the final solutions.
Furthermore, although problem~\eqref{eq:expected_risk_prob} is constrained, we can re-formulate it with variables $d_t := q_t - q_{t-1}$; this consequently replaces the current constraints with only non-negativity constraints $d_t \geq 0$.
Finally due to Assumption~\ref{ass:cdf_pdf_exists}, problem~\eqref{eq:expected_risk_prob} can be optimized via gradient descent.





\subsection{Learning and Optimizing the Data Requirement}
\label{sec:optimization_framework_learning}


Solving problem~\eqref{eq:expected_risk_prob} requires access to the true distribution $F(q)$, which we do not have in reality. 
In each round, given a current training data set $\dataset_{q_t}$ of $q_t$ points, we must estimate these distribution functions $F(q)$ and $f(q)$ and then incorporate them into our optimization problem. 
%We then use these estimated functions to solve our optimization problem.

%\JL{I moved things around to explain the procedure first and then compare to prior paper.}

Given a current data set $\dataset_{q_t}$, we may sample an increasing sequence of $R$ subsets
%partition it into $R$ consecutive subsets 
$\dataset_{q_t/R} \subset \dataset_{2q_t/R} \subset \cdots \subset \dataset_{q_t}$, fit our model to each subset, and compute the scores to obtain a data set of the learning curve $\set{R} := \{ (rq_t/R, V(\dataset_{rq_t/R})) \}_{r=1}^R$. In order to model the distribution of $D^*$, we can take $B$ bootstrap resamples of $\set{R}$ to fit a series of regression functions and obtain corresponding estimates $\{ \hat{D}_b \}_{b=1}^B$. \rebut{Given a set of estimates of the data requirement, we estimate the PDF via Kernel Density Estimation (KDE). Finally to fit the CDF, we numerically integrate the PDF. }



In our complete framework, LOC, we first estimate $F(q)$ and $f(q)$. We then use these models to solve problem~\eqref{eq:expected_risk_prob}.
Note that in the $t$-th round of collection, we fix the prior decision variables $q_1, \dots q_{t-1}$ constant. 
Finally, we collect data as determined by the optimal solution $q^*_t$ to problem~\eqref{eq:expected_risk_prob}.
Full details of the learning and optimization steps, including the complete Algorithm, are in Appendix~\ref{sec:app_opt}.





\subsection{Comparison to~\citet{mahmood2022howmuch}}
\label{sec:compare_vs_CVPR}





Our prediction model extends the previous approach of~\citet{mahmood2022howmuch}, who consider only point estimation of $D^*$.
They (i) build the set $\set{R}$, (ii) fit a parametric function $\hat{v}(q; \btheta)$ to $\set{R}$ via least-squares minimization, and (iii) solve for $\hat{D} = \argmin_{q} \{ q \;|\; \hat{v}(q; \btheta) \geq V^* \}$. 
They use several parametric functions from the neural scaling law literature, including the power law function (i.e.,  $\hat{v}(q;\btheta) := \theta_0 q^{\theta_1} + \theta_2$~\citep{mahmood2022howmuch,hoiem2021learning} where $\btheta := \{ \theta_0, \theta_1, \theta_2 \}$), and use an ad hoc correction factor obtained by trial and error on past tasks to help decrease the failure rate.
Instead, we take bootstrap samples of $\set{R}$ to fit multiple regression functions, estimate a distribution for $\hat{D}$, and incorporate them into our novel optimization model.
Finally, we show in the next two sections that our optimization problem has analytic solutions and extends to multiple sources. 







==> How Much More Data Should I Get for ArXiv/sections/problem_def.tex <==
\section{Main Problem}
\label{sec:data_collection_problem}














In this section, we give a motivating example before introducing the formal data collection problem.
We include a table of notation in Appendix~\ref{sec:app_notation}.


\textbf{Motivating Example.}
\emph{A startup is developing an object detector for use in autonomous vehicles within the next $T=5$ years.
Their model must achieve a mean Average Precision greater than $V^*=95\%$ on a pre-determined validation set or else they will lose an expected profit of $P = \$1,000,000$. 
Collecting training data requires employing drivers to record videos and annotators to label the data, where the marginal cost of obtaining each image is approximately $c = \$1$. 
In order to manage annual finances, the startup must plan how much data to collect at the beginning of each year.
}


Let $z \sim p(z)$ be data drawn from a distribution $p$. For instance, $z := (x, y)$ may correspond to images $x$ and labels $y$. 
Consider a prediction problem for which we train a model with a data set $\dataset$ of points sampled from $p(z)$. Let $V(\dataset)$ be a score function evaluating the model trained on $\dataset$. % (e.g., classification accuracy on a held-out validation set).


\textbf{Optimal Data Collection.}
We possess an initial data set $\dataset_{q_0} := \{z_i\}_{i=1}^{q_0}$ of $q_0$ points; we omit the subscript on $\dataset$ referring to its size when it is obvious.
Our problem is defined by a target score $V^* > V(\dataset_{q_0})$, a cost-per-sample $c$ of collection, a horizon of $T$ rounds, and a penalty $P$ for failure. 
At the end of each round $t \in \{1, \dots, T\}$, let $q_t$ be the current amount of data collected.
Our goal is to minimize the total collection cost while building a model that can achieve the target score:
%
\begin{align}\nonumber
     &\min_{q_1, \dots, q_T} \; c (q_T - q_0) + P \Ind \{ V(\dataset_{q_T}) < V^* \} \quad\;\;\;\;\;\;\;\;\;\; \st \; q_0 \leq q_1 \leq \cdots \leq q_T \\ \label{eq:formal_problem}
    =&\min_{q_1, \dots, q_T} \; c \sum_{t=1}^T(q_t - q_{t-1}) + P \Ind \{ V(\dataset_{q_T}) < V^* \} \quad\;\; \st \; q_0 \leq q_1 \leq \cdots \leq q_T
\end{align}
%
The collection cost is measured by the difference in data set size between the final and the 0-th round $c ( q_T - q_0 ) = c \sum_{t=1}^T(q_t - q_{t-1})$, 
Because we collect data iteratively over multiple rounds (see Figure \ref{fig:flowchart}), we break \eqref{eq:formal_problem} into the sum of differences per round. 
Specifically in each round, we 
%
\begin{enumerate}
    \item Decide to grow the data set to $q_t \geq q_{t-1}$ points by sampling $\hat\dataset := \{ \hat{z}_i \}_{i=1}^{q_t - q_{t-1}} \sim p(z)$.  Pay a cost $c (q_t - q_{t-1})$ and update $\dataset \gets \dataset \cup \hat\dataset$.
    
    \item Train the model and evaluate the score. If $V(\dataset) \geq V^*$, then terminate. 
    
    \item If $t = T$, then pay the penalty $P$ and terminate. Otherwise, repeat for the next round.
\end{enumerate}
%

%From the neural scaling law literature, 
The model score typically increases monotonically with data set size~\citep{hestness2017deep, rosenfeld2019constructive}. This means that the minimum cost strategy for~\eqref{eq:formal_problem} is to collect just enough data such that $V(\dataset_{q_T}) = V^*$.
%Let $D^*$ be the size of this data set.
%However, the exact minimum amount of data depends on the training dynamics and is not known a priori. 
We can estimate this minimum data requirement by modeling the score function as a stochastic process. 
Let $V_q := V(\dataset_q)$ and let $\{ V_q \}_{q \in \field{Z}_+}$ be a stochastic process whose indices represent training set sizes in different rounds. 
Then, collecting data in each round yields a sequence of subsampled data sets $\dataset_{q_{t-1}} \subset \dataset_{q_t}$ and 
their performances $V(\dataset_{q_t})$. 
The minimum data requirement is the stopping time
%
\begin{align}\label{eq:min_dat_req}
    D^* := \argmin_q \left\{q \;|\; V_q \geq V^* \right\}.
\end{align}
%
which is a random variable giving the first time that we pass the target. 
%which is the first time that we exceed the target score. 
Note that $q^*_1 = \cdots = q^*_T = D^*$ is a minimum cost solution to the optimal data collection problem, incurring a total cost $c (D^* - q_0)$\footnote{We assume that $c (D^* - q_0) < P$, since otherwise the optimal strategy would be to collect no data.}. 




Estimating $D^*$ using past observations of the learning curve is difficult since we have only $T$ rounds. Further,~\citet{mahmood2022howmuch} empirically show that small errors in fitting the learning curve can cause massive over- or under-collection. Thus, robust policies must capture the uncertainty of estimation.





==> How Much More Data Should I Get for ArXiv/sections/related.tex <==
\section{Related work}
\label{sec:setup_related_work}






\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.84\linewidth}
%\includegraphics[width=1\textwidth]{figures/FlowDiagramV5.pdf} 
\includegraphics[width=1\textwidth]{figures/FlowDiagramV6.pdf} 
\end{minipage}
    \vspace{-2mm}
    \caption{\label{fig:flowchart} In the optimal data collection problem, we iteratively determine the amount of data that we should have, pay to collect the additional data, and then re-evaluate our model. 
    Our approach, Learn-Optimize-Collect, optimizes for the minimum amount of data $q^*_t$ to collect.
    }
\end{center}
\vspace{-7mm}
\end{figure*}



\noindent \textbf{Neural Scaling Laws.}
\rebut{
According to the neural scaling law literature, the performance of a model on a validation set scales with the size of the training data set $q$ via a power law $V \propto \theta_0 q^{\theta_1}$~\citep{hestness2017deep, rosenfeld2019constructive, hoiem2021learning, bahri2021explaining, bisla2021theoretical, jones2003introduction, sun2017revisiting,  figueroa2012predicting, viering2021shape, zhai2021scaling}.
\citet{hestness2017deep} observe this property over vision, language, and audio tasks,~\citet{bahri2021explaining} develop a theoretical relationship under assumptions on over-parametrization and the Lipschitz continuity of the loss, model, and data, and~\citet{rosenfeld2019constructive} estimate power laws using smaller data sets and models to extrapolate future performance.
}
Multi-variate scaling laws have also been considered for some specific tasks, for example in transfer learning from synthetic to real data sets~\citep{mikami2021scaling}.
Finally,~\citet{mahmood2022howmuch} explore data collection by estimating the minimum amount of data needed to meet a given target performance over multiple rounds.
Our paper extends these prior studies by developing an optimization problem to minimize the expected total cost of data collected. Specifically, we incorporate the uncertainty in any regression estimate of data requirements and further generalize to multiple data sources with different costs.


\noindent \textbf{Active Learning.} 
%Sequential data collection is also modeled in active learning~\citep{cohn1993neural}, 
\rebut{
In active learning, a model sequentially collects data by selecting new subsets of an unlabeled data pool to label under a pre-determined labeling budget that replenishes after each round~\citep{settles2009active, sener2017active, yoo2019learning, sinha2019variational, mahmood2021low}. In contrast, our work focuses on systematically determining an optimal collection budget. After determining how much data to collect, we can use active learning techniques to collect the desired amount of data.
}



\noindent \textbf{Statistical Learning Theory.}
\rebut{
Theoretical analysis of the sample complexity of machine learning models is typically only tight asymptotically, but some recent work have empirically analyzed these relationships~\citep{jiang2020neurips, jiang2021methods}.
Particularly,~\citet{bisla2021theoretical} study generalization bounds for deep neural networks, provide empirical validation, and suggest using them to estimate data requirements. 
In contrast, our paper formally explores the consequences of collection costs on data requirements.
}





\noindent \textbf{Optimal Experiment Design.}
The topic of how to collect data, select samples, and design scientific experiments or controlled trials is well-studied in econometrics~\citep{smith1918standard, cohn1993neural, emery1998optimal}. 
For example,~\citet{bertsimas2015power} optimize the assignment of samples into control and trial groups to minimize inter-group variances.
Most recently,~\citet{carneiro2020optimal} optimize how many samples and covariates to collect in a statistical experiment by minimizing a treatment effect estimation error or maximizing $t$-test power.
However, our focus on industrial machine learning applications differs from experiment design by having target performance metrics and continual rounds of collection and modeling. 


==> How Much More Data Should I Get for ArXiv/sections/results.tex <==
\section{Empirical Results}
\label{sec:numerical_results}








We explore the data collection problem over two sets of experiments covering single-variate $K=1$ (Section~\ref{sec:optimization_framework}) and multi-variate $K = 2$ (Section~\ref{sec:multivariate}) problems. We consider image classification, segmentation, and object detection tasks. 
For every data set and task, LOC significantly reduces the number of instances where we fail to meet a data requirement $V^*$, while incurring a competitive cost with respect to the conventional baseline of na\"{i}vely estimating the data requirement~\citep{mahmood2022howmuch}. %slightly more than the minimum cost needed to meet the target.


In this section, we summarize the main results. We detail our data collection and experiment setup in Appendix~\ref{sec:app_experiments}. We expand our full results \rebut{and experiments with additional baselines} in Appendix~\ref{sec:app_experiment_results} .







\subsection{Data and Methods}





When $K=1$, the designer decides how much data to sample without controlling the type of data. We explore classification on CIFAR-10~\citep{krizhevsky2009learning}, CIFAR-100~\citep{krizhevsky2009learning}, and ImageNet~\citep{deng2009imagenet}, where we train ResNets~\citep{he2016deep} to meet a target validation accuracy. 
We explore semantic segmentation using Deeplabv3~\citep{chen2017rethinking} on BDD100K~\citep{yu2020bdd100k}, which is a large-scale driving data set, as well as Bird's-Eye-View (BEV) segmentation on nuScenes~\citep{nuscenes2019} using the `Lift Splat' architecture~\citep{liftsplat}; for both tasks, we desire a target mean intersection-over-union (IoU).
We explore 2-D object detection on PASCAL VOC~\citep{pascal-voc-2007, pascal-voc-2012} using SSD300~\citep{liu2016ssd}, where we evaluate mean average precision (mAP).



When $K=2$, the designer collects two types of data with different costs.
We first divide CIFAR-100 into two subsets containing data from the first and last 50 classes, respectively. 
Here, we assume that the first 50 classes are more expensive to collect than the last; this mimics a real-world scenario where collecting data for some classes (e.g., long-tail) is more expensive than others.
We then explore semi-supervised learning on BDD100K where the labeled subset of this data is more expensive than the unlabeled data; the cost difference between these two types is equal to the cost of data annotation.




We use a simulation model of the deep learning workflow following the procedure of~\citet{mahmood2022howmuch}, to approximate the true problem while simplifying the experiments (see Appendix~\ref{sec:app_experiments} for full details). 
To avoid repeatedly sampling data, re-training a model, and evaluating the score, each simulation uses a piecewise-linear approximation of a `ground truth' learning curve that returns model performance as a function of data set size.
In our problems, we initialize with $q_0 = 10\%$ of the full data set (we use $20\%$ for VOC). %and set a target score.
Then in each round, we solve for the amount of data to collect and then call the piecewise-linear learning curve to obtain the current score.


We compare LOC against the conventional estimation approach of~\citet{mahmood2022howmuch} who fit a regression model to the learning curve statistics, extrapolate the learning curve for larger data sets, and then solve for the minimum data requirement under this extrapolation.
There are many different regression models that can be used to fit learning curves~\citep{jones2003introduction, figueroa2012predicting, hestness2017deep, hoiem2021learning}. Since power laws are the most commonly studied approach in the neural scaling law literature, we focus on these.
In Appendix \ref{sec:app_experiment_alternate_regression_functions}, we show that our optimization approach can be incorporated with other regression models.












\subsection{Main Results}

We consider $T=1, 3, 5$ rounds and $V^* \in [V(\dataset_{q_0}) + 1, V(\dataset)]$ targets, where $\dataset$ is the entire data set.
We evaluate all methods on (i) the failure rate, which is how often the method fails to achieve the given $V^*$ within $T$ rounds, and (ii) the cost ratio, which is the suboptimality of an algorithm for solving problem \eqref{eq:expected_risk_prob}, i.e., $\bc^\tpose (\bq^*_T - \bq_0) / \bc^\tpose (\bD^* - \bq_0) - 1$. Note that the suboptimality does not count the penalty for failure since this would distort the average metrics.
For $K=1$, we also measure the ratio of points collected $q_T^* / D^*$.
Although there is a natural trade-off between low cost ratio (under-collecting) and failure rate (over-collecting), we emphasize that our goal is to have low cost but with zero chance of failure.






\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t1_V2/head_cifar10_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t1_V2/head_cifar100_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t1_V2/head_imagenet_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t1_V2/head_voc_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t1_V2/head_bdd100k_powerlawbootstrap_1_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t1_V2/head_liftsplatshoot_powerlawbootstrap_1_1.pdf}\end{minipage}
%
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t3_V2/head_cifar10_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t3_V2/head_cifar100_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t3_V2/head_imagenet_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t3_V2/head_voc_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t3_V2/head_bdd100k_powerlawbootstrap_3_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t3_V2/head_liftsplatshoot_powerlawbootstrap_3_1.pdf}\end{minipage}
%
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t5_V2/head_cifar10_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t5_V2/head_cifar100_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t5_V2/head_imagenet_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t5_V2/head_voc_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t5_V2/head_bdd100k_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.16\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_1d_t5_V2/head_liftsplatshoot_powerlawbootstrap_5_1.pdf}\end{minipage}
%
%
\vspace{-4mm}
\caption{\label{fig:head_to_head}
Mean $\pm$ standard deviation of 5 seeds of the ratio of data collected $q_T^* / D^*$ for different $V^*$. %We fix $c=1$ and $P=10^7$. 
The rows correspond to $T = 1, 3, 5$ and the columns to different data sets. The black line corresponds to collecting exactly the minimum data requirement. 
\rebut{LOC almost always remains slightly above the black line, meaning we rarely fail to meet the target.}
}
\end{center}
%\vspace{-7mm}
\vspace{-5mm}
\end{figure*}




\begin{table}[!t]
    %\centering
\begin{minipage}{0.66\linewidth}
\resizebox{\linewidth}{!}{
\begin{tabular}{clccccc}
\toprule
  & Data set &  $T$ & \multicolumn{2}{c}{Power Law Regression} & \multicolumn{2}{c}{LOC} \\ \cmidrule(lr){4-5}\cmidrule(lr){6-7}
  &          &      & Failure rate & Cost ratio & Failure rate & Cost ratio \\
\midrule
\multirow{9}{*}{\rotatebox[origin=c]{90}{Class.}}    
 & \multirow{3}{*}{CIFAR-10}    &  1 &   $100\%$ &             $-$ &        $\fir{60\%}$ &    $0.19$ \\
 &                              &  3 &   $ 95\%$ &          $0.00$ &        $\fir{32\%}$ &    $0.05$ \\
 &                              &  5 &   $ 86\%$ &          $0.00$ &        $\fir{29\%}$ &    $0.03$ \\
  \cmidrule{2-7} 
& \multirow{3}{*}{CIFAR-100}    &  1 &   $  56\%$ &          $0.12$ &        $\fir{4\%}$ &    $0.99$ \\
&                               &  3 &   $  48\%$ &          $0.10$ &        $\fir{3\%}$ &    $0.31$ \\
&                               &  5 &   $  48\%$ &          $0.10$ &        $\fir{2\%}$ &    $0.19$ \\
  \cmidrule{2-7} 
 & \multirow{3}{*}{Imagenet}    &  1 &   $  99\%$ &          $0.00$ &        $\fir{37\%}$ &    $0.49$ \\
 &                              &  3 &   $  75\%$ &          $0.01$ &        $\fir{ 5\%}$ &    $0.16$ \\
 &                              &  5 &   $  56\%$ &          $0.01$ &        $\fir{ 2\%}$ &    $0.10$ \\
 \midrule
  \multirow{6}{*}{\rotatebox[origin=c]{90}{Seg.}}    
  & \multirow{3}{*}{BDD100K}    &  1 &   $  77\%$ &          $0.03$ &        $\fir{12\%}$ &    $2.03$ \\
  &                             &  3 &   $  31\%$ &          $0.00$ &        $\fir{ 0\%}$ &    $0.72$ \\
  &                             &  5 &   $  23\%$ &          $0.01$ &        $\fir{ 0\%}$ &    $0.35$ \\
  \cmidrule{2-7} 
 & \multirow{3}{*}{nuScenes}    &  1 &   $  95\%$ &          $0.00$ &        $\fir{52\%}$ &    $0.16$ \\
 &                              &  3 &   $  71\%$ &          $0.01$ &        $\fir{ 0\%}$ &    $0.09$ \\
 &                              &  5 &   $  62\%$ &          $0.00$ &        $\fir{ 0\%}$ &    $0.04$ \\
 \midrule
 \multirow{3}{*}{\rotatebox[origin=c]{90}{Det.}}    
      & \multirow{3}{*}{VOC}    &  1 &   $  36\%$ &          $1.24$ &        $\fir{25\%}$ &      $0.56$ \\
      &                         &  3 &   $   8\%$ &          $0.88$ &        $\fir{ 0\%}$ &      $1.10$ \\
      &                         &  5 &   $   6\%$ &          $0.86$ &        $\fir{ 0\%}$ &      $0.84$ \\
\bottomrule
\end{tabular}
}
\end{minipage}
%
\hfill
%\begin{minipage}{0.5\linewidth}{}
\begin{minipage}{0.31\linewidth}
    \caption{Average cost ratio $\bc^\tpose (\bq^*_T - \bq_0) / \bc^\tpose (\bD^* - \bq_0) - 1$ and failure rate measured over a range of $V^*$ for each $T$ and data set. 
    We fix $c = 1$ and $P=10^7$ ($P=10^6$ for VOC and $P=10^8$ for ImageNet).
    The best performing failure rate for each setting is bolded. The cost ratio is measured only for instances that achieve $V^*$. LOC consistently reduces the average failure rate, often down to $0\%$, while keeping the average cost ratio almost always below $1$ (i.e., spending at most $2\times$ the optimal amount).}
    \label{tab:one_d_summary}
\end{minipage}
%\vspace{-5mm}
\vspace{-2mm}
\end{table}





\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t5_V2/sweepcost_cifar10_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t5_V2/sweepcost_cifar100_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t5_V2/sweepcost_imagenet_powerlawbootstrap_5_1.pdf}\end{minipage}
%
\vspace{-1em}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t5_V2/sweepcost_cifar10_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t5_V2/sweepcost_cifar100_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t5_V2/sweepcost_imagenet_powerlawbootstrap_5_1.pdf}\end{minipage}
%
\vspace{-1em}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t5_V2/sweepcost_voc_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t5_V2/sweepcost_bdd100k_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_costs/sim_1d_t5_V2/sweepcost_liftsplatshoot_powerlawbootstrap_5_1.pdf}\end{minipage}
%
\vspace{-1em}
%
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t5_V2/sweepcost_voc_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t5_V2/sweepcost_bdd100k_powerlawbootstrap_5_1.pdf}\end{minipage}
\begin{minipage}{0.3\linewidth}\includegraphics[width=1\textwidth]{figures/sweep_penalty/sim_1d_t5_V2/sweepcost_liftsplatshoot_powerlawbootstrap_5_1.pdf}\end{minipage}
%\vspace{-4mm}
%
\caption{\label{fig:sweep_cost_and_penalty}
Mean $\pm$ standard deviation of 5 seeds of the ratio of data collected $q_T^* / D^*$ for different $V^*$ and fixed $T=5$.
\emph{Rows 1 \& 3:} We sweep the cost parameter from $0.001$ to $1$ and fix $P=10^7$. 
\emph{Rows 2 \& 4:} We sweep the penalty parameter from $10^6$ to $10^9$ and fix $c = 1$. 
%We hold $c=1$ and $P=10^7$ fixed. The rows correspond to $T = 1, 3, 5$ and the columns to different data sets.
The dashed black line corresponds to collecting exactly the minimum data requirement.
See Appendix~\ref{sec:app_experiment_results} for all $T$.
}
\end{center}
\vspace{-6mm}
%\vspace{-9mm}
\end{figure*}






\textbf{The Value of Optimization over Estimation when $K=1$.~}
Figure~\ref{fig:head_to_head} compares LOC versus the corresponding power law regression baseline when $c=1$ and $P=10^7$ ($P=10^6$ for VOC and $P=10^8$ for ImageNet). If a curve is below the black line, then it failed to collect enough data to meet the target.
LOC consistently remains above this black line for most settings.
In contrast, even with up to $T=5$ rounds, collecting data based only on regression estimates leads to failure.



Table~\ref{tab:one_d_summary} aggregates the failure rates and cost ratios for each setting. 
To summarize, LOC fails at less than $10\%$ of instances for $12/18$ settings, whereas regression fails over $30\%$ for $15/18$ settings.
In particular, regression nearly always under-collects data when given a single $T=1$ round. Here, LOC reduces the risk of under-collecting by $40\%$ to $90\%$ over the baseline.
While this leads to a marginal increase in costs, our cost ratios are consistently less than $0.5$ for $12/18$ settings, meaning that we spend at most $50\%$ more than the true minimum cost.



We remark that previously,~\citet{mahmood2022howmuch} observed that incorrect regression estimates necessitated real machine learning workflows to collect data over multiple rounds. 
Instead, with LOC, we can make significantly improved data collection decisions even with a single round.





\textbf{Robustness to Cost and Penalty Parameters (see Appendix~\ref{sec:app_experiment_robustness} for details).~}
Figure~\ref{fig:sweep_cost_and_penalty} evaluates the ratio of points collected for $T=5$ when the cost and the penalty of the optimization problem are varied. Our algorithm is robust to variations in these parameters, as LOC retains the same shape and scale for almost every parameter setting and data set. %every data set except VOC. 
Further, LOC consistently remains above the horizontal $1$ line, showing that even after varying $c$ and $P$, we do not fail as frequently as the baseline.
Finally, validating Theorem~\ref{thm:t1_has_analytic_sol}, the penalty parameter $P$ provides natural control over the amount of data collected. As we increase $P$, the ratio of data collected increases consistently.








\begin{figure*}[!t]
\begin{center}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t5_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_5_1,0.5_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t5_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_5_1,0.2_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t5_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_5_1,0.1_0_100000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t5_V3/gmm_baseline_verysmallcifar100_powerlawbaseline_0_5_1,0.05_0_100000000.0.pdf} \end{minipage}
%
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t5_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_5_1,0.1_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t5_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_5_1,0.05_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t5_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_5_1,0.01_0_1000000000.0.pdf} \end{minipage}
\begin{minipage}{0.24\linewidth}\includegraphics[width=1\textwidth]{figures/head_to_head/sim_2d_t5_V3/gmm_baseline_bdd100kunlabeled_powerlawbaseline_0_5_1,0.005_0_1000000000.0.pdf} \end{minipage}
%
\vspace{-4mm}
\caption{\label{fig:two_d_head_to_head}
%\RRM{These results are raw and I am running another set with more trials.}
Mean $\pm$ standard deviation over 5 seeds of the cost ratio $\bc^\tpose (\bq^*_T - \bq_0) / \bc^\tpose (\bD^* - \bq_0) - 1$ and failure rate for different $V^*$, after removing $99$-th percentile outliers.
%We fix $c_0=1$, $P=10^{13}$, and $T=5$.
The columns correspond to scenarios where the first set $c^1$ costs increasingly more than the second $c^2$. 
%$c_1 = c_0/2, c_0/5, c_0/10, c_0/20$. 
See Appendix~\ref{sec:app_experiment_results} for all $T$.
}
\end{center}
\vspace{-5mm}
%\vspace{-8mm}
\end{figure*}














%\textbf{The Value of Optimization over Estimation when $K>1$ (Appendix~F.2).~}
\textbf{The Value of Optimization over Estimation when $K=2$ (Appendix~\ref{sec:app_experiment_k_equals_two}).~}
Figure~\ref{fig:two_d_head_to_head} compares LOC versus regression at $T=5$ with different costs, showing that we maintain a similar cost ratio to the regression alternative, but with lower failure rates. 
Table~\ref{tab:two_d_summary} aggregates failure rates and cost ratios for all settings, showing LOC consistently achieves lower failure rates for nearly all settings of $T$. 
When $T=5$, LOC also achieves lower cost ratios versus regression on CIFAR-100, meaning that with multiple rounds of collection, we can ensure meeting performance requirements while paying nearly the optimal amount of data.
However, solving the optimization problem is generally more difficult as $K$ increases, and we sometimes over-collect data by large margins.
In practice, these outliers can be identified from common sense (e.g., if a policy suggests collecting more data than we can reasonably afford, then we would not use the policy suggestion). 
Consequently, we report these results after removing the $99$-th percentile outliers with respect to total cost for both methods. 
Nonetheless, this challenge remains when $T=1$, particularly for CIFAR-100.





\begin{table}[t]
    \centering
\begin{minipage}{0.68\linewidth}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
   Data set & $T$ & Cost & \multicolumn{2}{c}{Power Law Regression} & \multicolumn{2}{c}{LOC} \\ \cmidrule(lr){4-5}\cmidrule(lr){6-7}
            &  &    & Failure rate & Cost ratio & Failure rate & Cost ratio \\
\midrule
 \multirow{12}{*}{\rotatebox[origin=c]{90}{CIFAR-100 (2 Types)}} 
    &  \multirow{4}{*}{1} & $(0.01, 0.0005)$&             $62\%$ &               0.89 &        $\fir{40\%}$ &             41.80 \\
    &                     & $(0.01, 0.001)$ &             $58\%$ &               1.19 &        $\fir{46\%}$ &             9.85 \\
    &                     & $(0.01, 0.002)$ &             $56\%$ &               1.55 &        $\fir{54\%}$ &             6.98 \\
    &                     & $(0.01, 0.005)$ &             $54\%$ &               1.65 &        $\fir{33\%}$ &             4.43 \\ \cmidrule{2-7}
    &  \multirow{4}{*}{3} & $(0.01, 0.0005)$&             $43\%$ &               3.47 &        $\fir{30\%}$ &             4.88 \\
    &                     & $(0.01, 0.001)$ &             $45\%$ &               1.22 &        $\fir{43\%}$ &             1.31 \\
    &                     & $(0.01, 0.002)$ &             $45\%$ &               1.47 &        $\fir{44\%}$ &             1.21 \\
    &                     & $(0.01, 0.005)$ &             $38\%$ &               1.31 &        $\fir{36\%}$ &             1.17 \\ \cmidrule{2-7}
    &  \multirow{4}{*}{5} & $(0.01, 0.0005)$&             $38\%$ &               3.31 &        $\fir{24\%}$ &             5.19 \\
    &                     & $(0.01, 0.001)$ &             $35\%$ &               1.22 &        $\fir{24\%}$ &             0.79 \\
    &                     & $(0.01, 0.002)$ &       $\fir{37\%}$ &               1.33 &        $     38\% $ &             0.90 \\
    &                     & $(0.01, 0.005)$ &             $36\%$ &               1.30 &        $\fir{24\%}$ &             0.82 \\
 \midrule
   \multirow{12}{*}{\rotatebox[origin=c]{90}{BDD100K (Semi-supervised)}} 
    &  \multirow{4}{*}{1} &  $(1, 0.005)$ &         $86\%$ &                 0.11 &        $\fir{44\%}$ &             7.02    \\
    &                     &   $(1, 0.01)$ &         $79\%$ &                 0.15 &        $\fir{30\%}$ &            13.47    \\
    &                     &   $(1, 0.05)$ &         $72\%$ &                 0.19 &        $\fir{49\%}$ &             1.02    \\
    &                     &    $(1, 0.1)$ &         $70\%$ &                 0.19 &        $\fir{65\%}$ &             0.40    \\ \cmidrule{2-7}
    &  \multirow{4}{*}{3} &  $(1, 0.005)$ &         $23\%$ &                 0.18 &        $\fir{ 7\%}$ &             1.20    \\
    &                     &   $(1, 0.01)$ &         $21\%$ &                 0.15 &        $\fir{ 7\%}$ &             2.57    \\
    &                     &   $(1, 0.05)$ &         $26\%$ &                 0.18 &        $\fir{23\%}$ &             0.50    \\
    &                     &    $(1, 0.1)$ &         $26\%$ &                 0.21 &        $\fir{30\%}$ &             0.15    \\ \cmidrule{2-7}
    &  \multirow{4}{*}{5} &  $(1, 0.005)$ &         $16\%$ &                 0.22 &        $\fir{ 2\%}$ &             1.91    \\
    &                     &   $(1, 0.01)$ &         $21\%$ &                 0.15 &        $\fir{ 2\%}$ &             0.86    \\
    &                     &   $(1, 0.05)$ &         $16\%$ &                 0.17 &        $\fir{ 9\%}$ &             0.27    \\
    &                     &    $(1, 0.1)$ &         $16\%$ &                 0.20 &        $\fir{ 7\%}$ &             0.32    \\
\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}{0.295\linewidth}
    \caption{
        Average cost ratio $\bc^\tpose (\bq^*_T - \bq_0) / \bc^\tpose (\bD^* - \bq_0) - 1$ and failure rate  over different $V^*$ for each $T$ and $\bc$, after removing $99$-th percentile outliers. We fix $P=10^{13}$ for CIFAR-100 and $P = 10^{8}$ for BDD100K.
        The best performing failure rate for each setting is bolded. The cost ratio is measured over instances that achieve $V^*$. 
        LOC consistently reduces the average failure rate, and for $T > 1$, preserves the cost ratio. 
        Further, LOC is more robust to uneven costs than regression.}
    \label{tab:two_d_summary}
\end{minipage}
%\vspace{-6mm}
\end{table}






==> How Much More Data Should I Get for ArXiv/sections/theory.tex <==
\section{Analytic Solutions for the $T=1$ Setting}
\label{sec:main_theory}



In this section, we explore analytic solutions for problem~\eqref{eq:expected_risk_prob}. 
The unobservable $D^*$ and sequential decision-making nature suggest this problem can be formulated as a Partially Observable Markov Decision Process (POMDP) with an infinite state and action space (see Appendix~\ref{sec:app_mdp_alternatives}), but such problems rarely permit exact solution methods~\citep{zhang2022dynamic}.
Nonetheless, we can derive exact solutions for the simple case of a single $T=1$ round, re-stated below
%
\begin{equation}\label{eq:expected_risk_prob_one_round}
    \min_{q_1} \; c(q_1 - q_0) + P(1 - F(q_1)) \qquad\qquad\qquad \st \; q_0 \leq q_1
\end{equation}
%
\begin{thm}\label{thm:t1_has_analytic_sol}
    Assume $F(q)$ is strictly increasing and continuous. If there exists $q_1 \geq q_0, \hat\epsilon \geq 0$ where  
    %
    \begin{align}\label{eq:expected_risk_prob_one_round_required_condition}
        \frac{c}{P} \leq \frac{F(q_1) - F(q_0)}{q_1 - q_0}, \qquad \hat\epsilon \leq 1 - F(q_0), \qquad P = c / f ( F^{-1}(1 - \hat\epsilon) )
    \end{align}
    %
    then there exists an $\epsilon \leq 1 - F(q_0)$ that satisfies
    $P = c / f ( F^{-1}(1 - \epsilon) )$ and
    an optimal solution to the corresponding problem~\eqref{eq:expected_risk_prob_one_round} is $q_1^* := F^{-1}(1 - \epsilon)$. 
    Otherwise, the optimal solution is $q_1^* := q_0$.
\end{thm}
%
When the penalty $P$ is specified via a failure risk $\epsilon$, the optimal solution to problem~\eqref{eq:expected_risk_prob_one_round} is equal to a quantile of the distribution of $D^*$. 
We defer the proof and some auxiliary results to Appendix~\ref{sec:app_proofs}.
%Because the proof requires several auxiliary results, we defer it to Appendix~\ref{sec:app_proofs}.




Theorem~\ref{thm:t1_has_analytic_sol} further provides guidelines on choosing values for the cost and penalty parameters.  
While $c$ is the dollar-value cost per-sample, which includes acquisition, cleaning, and annotation, $P$ can reflect their inherent regret or opportunity cost of failing to meet their target score. 
%Using Theorem~\ref{thm:t1_has_analytic_sol}, 
A designer can accept a risk $\epsilon$ of failing to collect enough data $\mathrm{Pr} \{ q^* < D^* \} = \epsilon$. 
From Theorem~\ref{thm:t1_has_analytic_sol}, their optimal strategy should be to collect $F^{-1}(1- \epsilon)$ points, which is also the optimal solution to problem~\eqref{eq:expected_risk_prob_one_round}.








==> sections/app_optimal_control.tex <==
\subsection{Optimal control framework}

In this section we introduce an optimal control perspective on our optimal data collection problem.

We define the state to be $q_t$, the amount of data that has been collected at time $t$. Within each round, a control $d_t \geq 0$ is chosen that corresponds to collecting $d_t$ new data points. At the end of each round, we pay a cost equal to $c d_t$ for some $c > 0$. We repeat this process for $T$ rounds and then we evaluate our model by computing $V_{q_T}$ and paying a penalty $P > 0$ if $V_{q_T} < V^*$. This describes an optimal control problem written as follows,
\begin{equation}
    \min_{d_0, \dots, d_{T-1}} \; \sum_{t=0}^{T-1}c d_t + P \Ind \{ V(\dataset_{q_T}) < V^* \} \quad\;\; \st \; d_t \geq 0,\textrm{ and }\:q_{t+1} = q_t + d_t.
\end{equation}
This is a stochastic control problem whose expected loss is written,
\begin{equation}
    \min_{d_0, \dots, d_{T-1}} \; \sum_{t=0}^{T-1}c d_t + P (1 - F(q_T)) \quad\;\; \st \; d_t \geq 0, \:\forall t.
\end{equation}
We can derive the control Hamiltonian,
\begin{equation}
    H = c d_t + \lambda_{t+1} d_t,
\end{equation}
where $\lambda_t$ is the costate. Pontryagin's maximum principle states that,
\begin{align*}
    q_{t+1} - q_t &= d_t,\\
    \lambda_{t+1} - \lambda_t &= 0,\\
    \lambda_T &= -Pf(q_T),\\
    d^*_t &= \arg\min_{d_t} H(q_t, d_t, \lambda_{t+1}).
\end{align*}
Solving the last equation gives us $\lambda_{t+1} = -c$, and using the fact that $\lambda_t$ is constant we recover $f(q_T) = c/P$. \JL{If you take the same $P^*$ as used in Theorem 1, you recover the same optimal choice for $q_T$. Further, you could add in $(1-F(q_{t+1}))$ to the per-round cost function to match our objective. But I'm not sure if this is necessary. I feel that we should recover an optimal policy if we correctly handle uncertainty in quantifying the distribution.}
